Structured factor copulas for modeling the systemic risk of European and United States banks

In this paper, we employ Credit Default Swaps (CDS) to model the joint and conditional distress probabilities of banks in Europe and the U.S. using factor copulas. We propose multi-factor, structured factor, and factor-vine models where the banks in the sample are clustered according to their geographic location. We find that within each region, the co-dependence between banks is best described using both, systematic and idiosyncratic, financial contagion channels. However, if we consider the banking system as a whole, then the systematic contagion channel prevails, meaning that the distress probabilities are driven by a latent global factor and region-specific factors. In all cases, the co-dependence structure of bank CDS spreads is highly correlated in the tail. The out-of-sample forecasts of several measures of systematic risk allow us to identify the periods of distress in the banking sector over the recent years including the COVID-19 pandemic, the interest rate hikes in 2022, and the banking crisis in 2023.

==> img/syst_idio_contagion.tex <==
\begin{figure}
    \begin{center}
    \begin{minipage}{.4\textwidth}
\begin{tikzpicture}
    \node (wa) [wa]  {$F$};
    \path (wa.south)+(-2,-1.2) node (m1f)[sensor] {$B_1$};
    \path (wa.south)+(0,-1.2) node (m2f)[sensor] {$B_2$}; 
    \path (wa.south)+(2,-1.2) node (m3f)[sensor] {$B_3$}; 
    \path [draw, <-,very thick] (m1f.north) -- node [above] {} (wa.250);
    \path [draw, <-,very thick] (m2f.north) -- node [above] {} (wa.270);
    \path [draw, <-,very thick] (m3f.north) -- node [above] {} (wa.290);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.4\textwidth}
\begin{tikzpicture}
    \node (sensor) [sensor] (b1) at (0,0) {$B_1$};
     \node (sensor) [sensor] (b2) at (2,0) {$B_2$};
     \node (sensor) [sensor] (b3) at (4,0) {$B_3$};

     \draw[->, very thick] (b1) to[bend left] node[left] {} (b2) ;
     \draw[->, very thick] (b1) to[bend right] node[left] {} (b3) ;
\end{tikzpicture}
\end{minipage}
\end{center}
    \caption{Systematic contagion (on the left) and idiosyncratic contagion (on the right).}
    \label{fig:label2}
\end{figure}

==> tables/desc_crude.tex <==
% latex table generated in R 4.3.0 by xtable 1.8-4 package
% Mon Jul 17 18:03:45 2023
\begin{table}[!htbp] 
\centering
\caption{Descriptive statistics for the CDS spreads.} 
\label{table:desc_crude}
\scalebox{0.8}{
\begin{threeparttable}
\begin{tabular}{rrrrrrrrrrrr}
  \hline
 & mean & Q2 & sd & skew & kurt & min & max & 1stACF & ADF(10) & LB(10) & ARCH(10) \\ 
  \hline
BCS & 94.98 & 82.32 & 51.27 & 0.92 & 3.65 & 5.45 & 278.64 & 0.99 & 0.04 & 0.00 & 0.00 \\ 
  BNP & 78.49 & 65.92 & 57.00 & 1.92 & 7.08 & 5.70 & 359.59 & 1.00 & 0.30 & 0.00 & 0.00 \\ 
  CS & 98.82 & 83.00 & 63.49 & 3.75 & 38.09 & 9.86 & 1082.15 & 0.98 & 0.01 & 0.00 & 0.00 \\ 
  GLE & 94.86 & 78.68 & 75.22 & 1.94 & 7.00 & 6.01 & 440.26 & 1.00 & 0.28 & 0.00 & 0.00 \\ 
  ISP & 137.49 & 108.28 & 103.97 & 1.82 & 6.27 & 5.76 & 627.82 & 1.00 & 0.34 & 0.00 & 0.00 \\ 
  SAN & 118.45 & 84.67 & 95.98 & 1.43 & 4.46 & 7.62 & 487.50 & 1.00 & 0.41 & 0.00 & 0.00 \\ 
  UBS & 76.50 & 61.64 & 54.80 & 1.50 & 5.69 & 4.55 & 361.68 & 1.00 & 0.01 & 0.00 & 0.00 \\ 
  UCG & 155.77 & 127.94 & 111.47 & 1.81 & 6.50 & 7.48 & 687.10 & 1.00 & 0.25 & 0.00 & 0.00 \\ 
  AXP & 74.59 & 43.67 & 88.85 & 3.82 & 20.01 & 8.53 & 685.75 & 1.00 & 0.01 & 0.00 & 0.00 \\ 
  BAC & 103.14 & 76.28 & 76.54 & 1.96 & 7.27 & 5.31 & 483.06 & 1.00 & 0.05 & 0.00 & 0.00 \\ 
  C & 114.77 & 82.80 & 90.03 & 2.40 & 10.96 & 7.44 & 665.53 & 1.00 & 0.02 & 0.00 & 0.00 \\ 
  GS & 115.41 & 93.16 & 71.68 & 1.89 & 6.82 & 20.90 & 545.14 & 0.99 & 0.01 & 0.00 & 0.00 \\ 
  JPM & 72.63 & 66.42 & 32.34 & 1.08 & 4.48 & 14.49 & 232.30 & 0.99 & 0.01 & 0.00 & 0.00 \\ 
  MS & 132.88 & 89.34 & 114.34 & 3.05 & 19.62 & 17.83 & 1360.00 & 0.98 & 0.01 & 0.00 & 0.00 \\ 
  WFC & 72.03 & 60.51 & 37.87 & 1.79 & 8.79 & 6.40 & 304.12 & 0.99 & 0.01 & 0.00 & 0.00 \\ 
   \hline
\end{tabular}
\begin{tablenotes}
\item {\footnotesize\textbf{Notes:} The table reports the descriptive statistics for the CDS spreads. 1stACF is the first-order autocorrelation, ADF($m$) is the $p$-value for the Augmented Dickey-Fuller test with $m$ lags,
the LB($k$) is  the $p$-value for the Ljung-Box test for  autocorrelation of $k$ lags,
and  ARCH($l$) is the $p$-value for the test for ARCH effects with $l$ lags. The data is from January 1st, 2007  to May 1st, 2023.}
    \end{tablenotes}
      \end{threeparttable}  
}

\end{table}


==> tables/insample_bics_berlin.tex <==
\begin{table}[!htbp] 
\centering
\caption{In-sample Bayesian Information Criteria.} 
\label{table:BIC}
\scalebox{0.6}{
\begin{threeparttable}
\begin{tabular}{rccccc}
  \hline
 & Subsample 1 & Subsample 2 & Subsample 3 & Subsample 4 & Full sample \\ 
 & Jan 2007 - Dec 2010 & Jan 2011 - Dec 2014 & Jan 2015 - Dec 2019 & Jan 2020 - May 2023 & Jan 2007 - May 2023 \\ \hline
 \multicolumn{5}{l}{U.S.\ banks} \\
  One-factor &  -4200.99 & -5830.27 & -7006.16 & \sh -6170.19 & -22622.88 \\ 
  Two-factor & -4182.95 & -5803.62 & -6979.97 & -6098.57 & -22610.04 \\ 
  Factor-Vine & \sh -4455.18 & \sh -5834.02 & \sh -7017.22 & -6161.97 & \sh -22698.24\\ 
 \hline 
 \multicolumn{5}{l}{European banks} \\
  One-factor & -7359.31 & -8951.08 & -7829.39 & -6725.13 & -30878.72 \\ 
  Two-factor & -7407.53 & -8884.31 & -7873.32 & -6980.22 & -32215.13 \\ 
  Factor-Vine & \sh -7446.67 & \sh -9125.10 & \sh -8646.63 & \sh -7096.86 & \sh -32670.12 \\ 
\hline   
 \multicolumn{5}{l}{U.S.\ and European banks} \\
  One-factor & -9175.17 & -11433.56 & -10301.33 & -10392.73 & -41131.21 \\ 
  Two-factor & -11744.15 & -14924.44 & -14964.80 & -13293.54 & -54773.96 \\ 
  Bi-factor & \sh -12016.55 & \sh -15322.08 & \sh -15809.10 & \sh -13429.70 & \sh -56212.63 \\ 
  Nested-factor & -11761.48 & -15202.06 & -15191.11 & -13472.43 & -54336.74 \\ 
  Factor-Vine & -11563.51 & -14732.43 & -15498.63 & -13346.46 & -53731.25 \\  \hline  
\end{tabular}
\begin{tablenotes}
\item {\footnotesize\textbf{Notes:} The table reports the in-sample Bayesian Information Criteria (BIC) for four subperiods and the full sample.}
    \end{tablenotes}
      \end{threeparttable}  
}

\end{table}


==> tables/insample_loglik.tex <==
\begin{table}[!htbp] 
\centering
\caption{In-sample log likelihoods.} 
\label{table:LLH}
\scalebox{0.8}{
\begin{threeparttable}
\begin{tabular}{rccccc}
  \hline
 & Subsample 1 & Subsample 2 & Subsample 3 & Subsample 4 & Full sample \\ 
 & Jan  07 - Dec  10 & Jan  11 - Dec  14 & Jan  15 - Dec  19 & Jan  20 - May  23 & Jan 07- May  23 \\ \hline
 \multicolumn{5}{l}{US banks} \\
  One-factor & 2148.77 & 2963.76 & 3551.71 & 3133.74 & 11369.69 \\ 
  Two-factor & 2163.88 & 2974.76 & 3562.93 & 3146.57 & 11392.39 \\ 
  Factor-Vine &\sh 2296.55 & \sh 2989.95 & \sh 3585.02 & \sh 3157.42 & \sh 11440.65 \\ 
\hline 
 \multicolumn{5}{l}{Euro banks} \\
   One-factor & 3734.82 & 4531.12 & 3970.27 & 3418.16 & 15505.93 \\ 
  Two-factor & 3786.51 & 4553.30 & 4047.81 & 3601.29 & 16232.38 \\ 
  Factor-Vine & \sh 3806.08 & \sh 4656.33 & \sh 4413.63 & \sh 3635.29 & \sh 16443.24 \\   \hline 
 \multicolumn{5}{l}{US and Euro banks} \\
  One-factor & 4691.02 & 5820.99 & 5254.87 & 5300.60 & 20690.42 \\ 
  Two-factor & 6051.36 & 7628.95 & 7656.07 & 6820.49 & 27603.33 \\ 
  Bi-factor & \sh 6201.35 & \sh 7845.14 & \sh 8102.54 & \sh 6892.05 & \sh 28343.47 \\ 
  Nested-factor & 5997.97 & 7719.13 & 7713.65 & 6854.35 & 27309.83 \\ 
  Factor-Vine & 5961.04 & 7546.84 & 7919.52 & 6840.00 & 27098.62 \\  \hline  

\end{tabular}
\begin{tablenotes}
\item {\footnotesize\textbf{Notes:} The table reports the in-sample log likelihoods for four subperiods and the full sample. The data is  from January 1st, 2007  to May 1st, 2023. We calculate the log likelihood of the factor copulas  at the posterior modes of the copula model parameters}
    \end{tablenotes}
      \end{threeparttable}  
}

\end{table}


==> tables/marginals_FS.tex <==
% latex table generated in R 4.3.0 by xtable 1.8-4 package
% Thu Sep 21 16:35:31 2023
\begin{table}[!htbp] 
\centering
\caption{Estimation results for the marginals. } 
\scalebox{0.8}{
\begin{threeparttable}
\begin{tabular}{rlllllllllll}
  \hline
 & $\mu$ & $\phi_1$ & $\phi_2$ & $\phi_3$ & $\phi_4$ & $\omega$ & $\alpha$ & $\beta$ & $\gamma$ & $\xi$ & $\nu$ \\ 
  \hline
BCS & -0.062 & 0.134 & 0.009 & 0.012 & -0.030 & 0.492 & 0.214 & 0.798 & -0.026 & 1.018 & 3.810 \\ 
   & (0.051) & (0.018) & (0.016) & (0.016) & (0.014) & (0.13) & (0.032) & (0.025) & (0.032) & (0.019) & (0.238) \\ 
  BNP & 0.016 & 0.117 & -0.005 & 0.000 & -0.034 & 0.435 & 0.196 & 0.834 & -0.060 & 1.059 & 4.069 \\ 
   & (0.055) & (0.016) & (0.015) & (0.015) & (0.014) & (0.225) & (0.036) & (0.034) & (0.031) & (0.021) & (0.319) \\ 
  CS & 0.003 & 0.146 & 0.010 & -0.007 & 0.007 & 0.534 & 0.293 & 0.765 & -0.117 & 1.031 & 3.641 \\ 
   & (0.054) & (0.017) & (0.015) & (0.015) & (0.014) & (0.172) & (0.054) & (0.039) & (0.048) & (0.019) & (0.216) \\ 
  GLE & -0.029 & 0.126 & -0.001 & -0.004 & -0.028 & 0.631 & 0.217 & 0.808 & -0.071 & 1.040 & 4.027 \\ 
   & (0.056) & (0.017) & (0.016) & (0.015) & (0.014) & (0.22) & (0.036) & (0.03) & (0.032) & (0.019) & (0.294) \\ 
  ISP & -0.027 & 0.165 & -0.001 & -0.010 & -0.017 & 0.596 & 0.202 & 0.809 & -0.024 & 1.028 & 3.874 \\ 
   & (0.064) & (0.017) & (0.015) & (0.016) & (0.015) & (0.197) & (0.038) & (0.031) & (0.034) & (0.022) & (0.248) \\ 
  SAN & -0.042 & 0.159 & -0.005 & -0.025 & -0.013 & 0.507 & 0.184 & 0.834 & -0.065 & 1.028 & 4.696 \\ 
   & (0.061) & (0.017) & (0.016) & (0.015) & (0.015) & (0.172) & (0.032) & (0.025) & (0.027) & (0.02) & (0.383) \\ 
  UBS & -0.019 & 0.076 & 0.022 & 0.009 & -0.029 & 0.524 & 0.197 & 0.840 & -0.115 & 1.030 & 4.033 \\ 
   & (0.056) & (0.018) & (0.014) & (0.015) & (0.015) & (0.166) & (0.036) & (0.029) & (0.03) & (0.021) & (0.286) \\ 
  UCG & -0.086 & 0.182 & 0.003 & -0.011 & -0.019 & 0.565 & 0.240 & 0.799 & -0.078 & 1.007 & 4.027 \\ 
   & (0.064) & (0.015) & (0.015) & (0.015) & (0.014) & (0.246) & (0.041) & (0.033) & (0.036) & (0.021) & (0.285) \\ 
  AXP & -0.095 & 0.076 & 0.080 & 0.021 & -0.001 & 0.130 & 0.139 & 0.858 & 0.004 & 1.005 & 4.489 \\ 
   & (0.05) & (0.025) & (0.017) & (0.018) & (0.018) & (0.205) & (0.054) & (0.068) & (0.026) & (0.017) & (0.314) \\ 
  BAC & -0.079 & 0.175 & 0.038 & -0.012 & -0.018 & 0.391 & 0.215 & 0.814 & -0.059 & 1.033 & 3.528 \\ 
   & (0.051) & (0.018) & (0.016) & (0.015) & (0.012) & (0.123) & (0.032) & (0.027) & (0.034) & (0.02) & (0.195) \\ 
  C & -0.062 & 0.165 & 0.057 & -0.013 & -0.024 & 0.381 & 0.264 & 0.788 & -0.103 & 1.058 & 3.869 \\ 
   & (0.05) & (0.019) & (0.015) & (0.015) & (0.015) & (0.137) & (0.048) & (0.037) & (0.041) & (0.021) & (0.246) \\ 
  GS & -0.069 & 0.160 & 0.069 & -0.015 & -0.032 & 0.454 & 0.279 & 0.772 & -0.102 & 1.030 & 3.396 \\ 
   & (0.046) & (0.018) & (0.016) & (0.016) & (0.015) & (0.173) & (0.052) & (0.044) & (0.044) & (0.019) & (0.196) \\ 
  JPM & -0.029 & 0.128 & 0.046 & -0.008 & -0.021 & 0.382 & 0.214 & 0.826 & -0.082 & 1.049 & 3.527 \\ 
   & (0.049) & (0.017) & (0.015) & (0.015) & (0.015) & (0.222) & (0.065) & (0.06) & (0.036) & (0.021) & (0.224) \\ 
  MS & -0.102 & 0.088 & 0.057 & 0.005 & -0.031 & 0.449 & 0.254 & 0.788 & -0.084 & 1.028 & 3.524 \\ 
   & (0.048) & (0.02) & (0.015) & (0.016) & (0.014) & (0.139) & (0.038) & (0.032) & (0.038) & (0.019) & (0.2) \\ 
  WFC & -0.041 & 0.157 & 0.044 & 0.011 & -0.032 & 0.311 & 0.218 & 0.827 & -0.088 & 1.074 & 3.803 \\ 
   & (0.047) & (0.022) & (0.017) & (0.017) & (0.016) & (0.137) & (0.051) & (0.041) & (0.034) & (0.02) & (0.269) \\ 
   \hline
\end{tabular}
\begin{tablenotes}
\item {\footnotesize\textbf{Notes:} The table reports the estimated parameters and standard errors
             (in parenthesis) for AR(4)-GJR-GARCH(1,1)
             model with skew-$t$ errors from January 1st, 2007 to May 1st, 2023.}
    \end{tablenotes}
      \end{threeparttable} 
}

\label{table:marginals}
\end{table}


==> tables/numberofmissing.tex <==
\begin{table}[!htbp] 
\centering
\caption{Missing values.}\label{table:numberofmissing}
\scalebox{0.8}{
\begin{threeparttable}
  \begin{tabular}{rrrrrrrrrrrrrrrr}
  \hline
 & BCS & BNP & CS & GLE & ISP & SAN & UBS & UCG & AXP & BAC & C & GS & JPM & MS & WFC \\ 
  \hline
Number & 30 & 0& 31 & 0 & 55& 0 & 1 & 0& 237& 9 & 3 & 158 & 1 & 58& 35 \\ 
\%   & 0.73 & 0.00 & 0.75 & 0.00 & 1.34 & 0.00 & 0.02 & 0.00 & 5.77 & 0.22 & 0.07 & 3.84 & 0.02 & 1.41 & 0.85 \\ 
   \hline
\end{tabular}
\begin{tablenotes}
\item {\footnotesize\textbf{Notes:} The table reports the number of missing CDS data values for each asset for the period from January 1st, 2007 to May 1st, 2023. Top row reports the number of total observations, and bottom row reports the corresponding proportion (in \%).}
    \end{tablenotes}
      \end{threeparttable}  
      }
\end{table}




==> tables/residuals_FS.tex <==
% latex table generated in R 4.3.0 by xtable 1.8-4 package
% Thu Sep 21 16:38:14 2023
\begin{table}[!htbp]
\centering
\caption{Descriptive statistics for marginal model residuals.} 
\scalebox{0.8}{
\begin{threeparttable}
\begin{tabular}{rrrrrrrrrrrrrr}
  \hline
 & mean & Q2 & sd & skew & kurtosis & min & max & LB(10) & ARCH(10) & KS & AD & DD & T \\ 
  \hline
BCS & 0.02 & 0.00 & 0.98 & 0.10 & 9.52 & -10.30 & 7.13 & 0.18 & 0.89 & 0.13 & 0.29 & 0.35 & 4110\\ 
  BNP & 0.01 & -0.02 & 0.99 & 0.19 & 8.34 & -9.69 & 6.38 & 0.12 & 0.76 & 0.57 & 0.44 & 0.72 & 4110\\ 
  CS & 0.02 & -0.00 & 0.99 & 0.53 & 7.97 & -4.95 & 7.17 & 0.03 & 0.17 & 0.13 & 0.19 & 0.52 & 4110\\ 
  GLE & 0.01 & -0.01 & 0.98 & 0.27 & 8.35 & -9.11 & 7.38 & 0.04 & 0.90 & 0.29 & 0.31 & 0.55 & 4110\\ 
  ISP & 0.01 & -0.01 & 0.98 & 0.21 & 7.42 & -7.47 & 7.23 & 0.53 & 0.28 & 0.69 & 0.82 & 0.62 & 4110\\ 
  SAN & 0.01 & -0.01 & 0.98 & 0.16 & 5.61 & -5.13 & 7.38 & 0.09 & 0.65 & 0.28 & 0.36 & 0.46 & 4110\\ 
  UBS & 0.01 & -0.01 & 0.98 & 0.04 & 7.92 & -9.31 & 6.36 & 0.04 & 0.86 & 0.66 & 0.62 & 0.49 & 4110\\ 
  UCG & 0.02 & 0.01 & 0.97 & 0.23 & 6.15 & -5.26 & 6.76 & 0.05 & 0.63 & 0.19 & 0.30 & 0.35 & 4110\\ 
  AXP & 0.02 & 0.02 & 1.03 & 0.17 & 8.02 & -9.75 & 7.15 & 0.82 & 0.63 & 0.02 & 0.06 & 0.00 & 4110\\ 
  BAC & 0.02 & -0.00 & 1.03 & 0.13 & 16.54 & -11.46 & 10.81 & 0.66 & 0.00 & 0.08 & 0.18 & 0.31 & 4110\\ 
  C & 0.02 & -0.02 & 1.00 & 0.30 & 10.15 & -8.22 & 9.81 & 0.05 & 0.92 & 0.08 & 0.15 & 0.32 & 4110\\ 
  GS & 0.03 & -0.01 & 1.04 & 2.25 & 36.06 & -5.86 & 16.82 & 0.50 & 0.88 & 0.03 & 0.14 & 0.39 & 4110\\ 
  JPM & 0.01 & -0.02 & 0.98 & 0.22 & 11.76 & -9.58 & 8.56 & 0.32 & 0.74 & 0.10 & 0.22 & 0.61 & 4110\\ 
  MS & 0.02 & -0.00 & 1.01 & 0.20 & 13.20 & -9.93 & 10.22 & 0.03 & 0.96 & 0.03 & 0.04 & 0.00 & 4110\\ 
  WFC & 0.02 & -0.01 & 0.98 & 0.92 & 9.30 & -5.62 & 8.65 & 0.15 & 0.00 & 0.13 & 0.17 & 0.36 & 4110\\ 
   \hline
\end{tabular}
\begin{tablenotes}
\item {\footnotesize\textbf{Notes:} The table reports the descriptive statistics for the AR(4)-GJR-GARCH(1,1) model with skew-$t$ errors residuals. 
 LB($k$) is  the $p$-value for the Ljung-Box test for  autocorrelation of $k$ lags,
  ARCH($l$) is the $p$-value for the test for ARCH effects with $l$ lags, KS is the $p$-value for the Kolmogorov–Smirnov test, AD is the $p$-value for the Anderson-Darling test, and DD is the $p$-value for the data-driven smooth test for uniformity. The data is from January 1st, 2007  to May 1st, 2023.}
    \end{tablenotes}
      \end{threeparttable}
}
\label{table:residuals}
\end{table}


==> tables/systemic.tex <==
% US
\begin{table}[!htbp] 
\centering
\caption{Probability of Distress for U.S.\ banks.} 
\scalebox{0.8}{
\begin{tabular}{rrrrrrrr}
  \hline
 & AXP & BAC & C & GS & JPM & MS & WFC \\ 
  \hline
2019-02-28 & 0.01 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.06 \\ 
  2019-03-28 & 0.03 & 0.00 & 0.01 & 0.02 & 0.01 & 0.06 & 0.07 \\ 
  2019-04-26 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.02 \\ 
  2019-05-29 & 0.02 & 0.03 & 0.05 & 0.02 & 0.01 & 0.04 & 0.37 \\ 
  2019-06-26 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & 0.04 \\ 
  2019-07-29 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 \\ 
  2019-09-10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\ 
  2019-10-08 & 0.03 & 0.01 & 0.01 & 0.02 & 0.01 & 0.02 & 0.11 \\ 
  2019-11-06 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\ 
  2019-12-09 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\ 
  2020-01-13 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\ 
  2020-02-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\ 
  2020-03-11 & 0.54 & 0.44 & 0.58 & 0.56 & 0.69 & 0.61 & 0.68 \\ 
  2020-04-08 & 0.81 & 0.47 & 0.66 & 0.51 & 0.62 & 0.43 & 0.90 \\ 
  2020-05-06 & 0.41 & 0.09 & 0.44 & 0.24 & 0.41 & 0.13 & 0.45 \\ 
  2020-06-03 & 0.06 & 0.06 & 0.08 & 0.05 & 0.13 & 0.03 & 0.22 \\ 
  2020-07-01 & 0.02 & 0.10 & 0.16 & 0.13 & 0.32 & 0.05 & 0.35 \\ 
  2020-08-04 & 0.00 & 0.02 & 0.03 & 0.13 & 0.05 & 0.02 & 0.16 \\ 
  2020-09-02 & 0.00 & 0.00 & 0.00 & 0.14 & 0.01 & 0.00 & 0.03 \\ 
  2020-10-05 & 0.01 & 0.01 & 0.02 & 0.19 & 0.04 & 0.02 & 0.13 \\ 
  2020-11-03 & 0.00 & 0.01 & 0.02 & 0.07 & 0.02 & 0.01 & 0.10 \\ 
  2020-12-04 & 0.00 & 0.07 & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 \\ 
  2021-01-14 & 0.01 & 0.01 & 0.00 & 0.28 & 0.01 & 0.00 & 0.01 \\ 
  2021-02-11 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 \\ 
  2021-03-11 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.02 \\ 
  2021-04-08 & 0.02 & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 & 0.04 \\ 
  2021-05-06 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 \\ 
  2021-06-03 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 & 0.01 \\ 
  2021-07-01 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 \\ 
  2021-07-29 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.02 & 0.00 \\ 
  2021-08-26 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.00 \\ 
  2021-09-23 & 0.00 & 0.03 & 0.01 & 0.01 & 0.03 & 0.03 & 0.01 \\ 
  2021-10-22 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.02 & 0.01 \\ 
  2021-11-19 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 & 0.01 \\ 
  2022-01-03 & 0.00 & 0.02 & 0.02 & 0.01 & 0.02 & 0.02 & 0.01 \\ 
  2022-01-31 & 0.00 & 0.16 & 0.09 & 0.08 & 0.17 & 0.18 & 0.08 \\ 
  2022-02-28 & 0.00 & 0.32 & 0.27 & 0.35 & 0.35 & 0.20 & 0.23 \\ 
  2022-03-28 & 0.04 & 0.44 & 0.49 & 0.23 & 0.46 & 0.37 & 0.27 \\ 
  2022-04-28 & 0.81 & 0.84 & 0.85 & 0.58 & 0.89 & 0.72 & 0.72 \\ 
  2022-05-27 & 0.84 & 0.55 & 0.56 & 0.49 & 0.61 & 0.51 & 0.54 \\ 
  2022-06-28 & 0.32 & 0.84 & 0.85 & 0.86 & 0.81 & 0.81 & 0.80 \\ 
  2022-07-28 & 0.03 & 0.31 & 0.31 & 0.42 & 0.40 & 0.29 & 0.27 \\ 
  2022-08-25 & 0.01 & 0.10 & 0.08 & 0.15 & 0.10 & 0.12 & 0.06 \\ 
  2022-09-22 & 0.09 & 0.66 & 0.62 & 0.58 & 0.69 & 0.56 & 0.61 \\ 
  2022-10-20 & 0.03 & 0.81 & 0.81 & 0.74 & 0.77 & 0.74 & 0.64 \\ 
  2022-11-17 & 0.15 & 0.11 & 0.14 & 0.13 & 0.07 & 0.24 & 0.05 \\ 
  2023-01-04 & 0.02 & 0.09 & 0.06 & 0.06 & 0.08 & 0.23 & 0.05 \\ 
  2023-02-01 & 0.00 & 0.01 & 0.01 & 0.02 & 0.01 & 0.02 & 0.01 \\ 
  2023-03-01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 \\ 
  2023-03-29 & 0.04 & 0.43 & 0.24 & 0.18 & 0.26 & 0.22 & 0.40 \\ 
   \hline
\end{tabular}
}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Joint Probability of Distress for U.S.\ banks.} 
\scalebox{0.8}{
\begin{tabular}{rrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\ 
  \hline
2019-02-28 & 0.07 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-03-28 & 0.12 & 0.04 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2019-04-26 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-05-29 & 0.39 & 0.08 & 0.04 & 0.02 & 0.01 & 0.01 & 0.00 \\ 
  2019-06-26 & 0.05 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-07-29 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-09-10 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-10-08 & 0.14 & 0.04 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 \\ 
  2019-11-06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-12-09 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-01-13 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-02-11 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-03-11 & 0.89 & 0.79 & 0.69 & 0.60 & 0.50 & 0.39 & 0.23 \\ 
  2020-04-08 & 0.96 & 0.88 & 0.75 & 0.64 & 0.52 & 0.40 & 0.25 \\ 
  2020-05-06 & 0.70 & 0.52 & 0.39 & 0.27 & 0.17 & 0.10 & 0.04 \\ 
  2020-06-03 & 0.30 & 0.15 & 0.09 & 0.05 & 0.03 & 0.02 & 0.00 \\ 
  2020-07-01 & 0.48 & 0.29 & 0.17 & 0.11 & 0.06 & 0.03 & 0.00 \\ 
  2020-08-04 & 0.22 & 0.10 & 0.04 & 0.02 & 0.01 & 0.00 & 0.00 \\ 
  2020-09-02 & 0.15 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-10-05 & 0.25 & 0.10 & 0.04 & 0.02 & 0.01 & 0.00 & 0.00 \\ 
  2020-11-03 & 0.14 & 0.05 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 \\ 
  2020-12-04 & 0.09 & 0.03 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2021-01-14 & 0.28 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-02-11 & 0.03 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-03-11 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-04-08 & 0.07 & 0.03 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2021-05-06 & 0.03 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-06-03 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-01 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-29 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-08-26 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-09-23 & 0.07 & 0.03 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2021-10-22 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-11-19 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-03 & 0.06 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-31 & 0.33 & 0.18 & 0.12 & 0.07 & 0.04 & 0.02 & 0.00 \\ 
  2022-02-28 & 0.57 & 0.40 & 0.30 & 0.22 & 0.15 & 0.07 & 0.00 \\ 
  2022-03-28 & 0.70 & 0.54 & 0.42 & 0.32 & 0.21 & 0.11 & 0.02 \\ 
  2022-04-28 & 0.97 & 0.94 & 0.89 & 0.83 & 0.75 & 0.62 & 0.40 \\ 
  2022-05-27 & 0.93 & 0.79 & 0.68 & 0.58 & 0.49 & 0.38 & 0.24 \\ 
  2022-06-28 & 0.97 & 0.93 & 0.89 & 0.84 & 0.77 & 0.64 & 0.25 \\ 
  2022-07-28 & 0.64 & 0.47 & 0.35 & 0.27 & 0.19 & 0.10 & 0.01 \\ 
  2022-08-25 & 0.28 & 0.14 & 0.09 & 0.06 & 0.03 & 0.02 & 0.00 \\ 
  2022-09-22 & 0.87 & 0.77 & 0.69 & 0.60 & 0.49 & 0.33 & 0.06 \\ 
  2022-10-20 & 0.94 & 0.88 & 0.82 & 0.75 & 0.65 & 0.48 & 0.02 \\ 
  2022-11-17 & 0.40 & 0.20 & 0.12 & 0.08 & 0.05 & 0.03 & 0.01 \\ 
  2023-01-04 & 0.30 & 0.12 & 0.07 & 0.04 & 0.03 & 0.01 & 0.00 \\ 
  2023-02-01 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-03-01 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-03-29 & 0.59 & 0.43 & 0.31 & 0.23 & 0.14 & 0.07 & 0.01 \\
   \hline
\end{tabular}
}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Expected Proportion in Distress for U.S.\ banks.}
\scalebox{0.8}{
\begin{tabular}{rrrrrrrr}
  \hline
 & AXP & BAC & C & GS & JPM & MS & WFC \\ 
  \hline
2019-02-28 & 0.33 & 0.66 & 0.51 & 0.36 & 0.45 & 0.42 & 0.21 \\ 
  2019-03-28 & 0.32 & 0.72 & 0.59 & 0.45 & 0.58 & 0.30 & 0.28 \\ 
  2019-04-26 & 0.29 & 0.64 & 0.52 & 0.35 & 0.45 & 0.35 & 0.22 \\ 
  2019-05-29 & 0.45 & 0.58 & 0.47 & 0.60 & 0.68 & 0.48 & 0.20 \\ 
  2019-06-26 & 0.38 & 0.39 & 0.37 & 0.47 & 0.44 & 0.39 & 0.21 \\ 
  2019-07-29 & 0.38 & 0.42 & 0.38 & 0.41 & 0.44 & 0.27 & 0.22 \\ 
  2019-09-10 & 0.22 & 0.40 & 0.42 & 0.35 & 0.33 & 0.32 & 0.25 \\ 
  2019-10-08 & 0.33 & 0.59 & 0.57 & 0.50 & 0.53 & 0.44 & 0.23 \\ 
  2019-11-06 & 0.28 & 0.43 & 0.50 & 0.38 & 0.37 & 0.34 & 0.24 \\ 
  2019-12-09 & 0.26 & 0.43 & 0.36 & 0.35 & 0.34 & 0.30 & 0.21 \\ 
  2020-01-13 & 0.20 & 0.43 & 0.40 & 0.37 & 0.32 & 0.36 & 0.22 \\ 
  2020-02-11 & 0.22 & 0.43 & 0.33 & 0.40 & 0.33 & 0.32 & 0.21 \\ 
  2020-03-11 & 0.78 & 0.88 & 0.81 & 0.82 & 0.75 & 0.79 & 0.76 \\ 
  2020-04-08 & 0.71 & 0.88 & 0.80 & 0.86 & 0.80 & 0.89 & 0.68 \\ 
  2020-05-06 & 0.53 & 0.84 & 0.57 & 0.70 & 0.58 & 0.78 & 0.56 \\ 
  2020-06-03 & 0.45 & 0.59 & 0.56 & 0.59 & 0.44 & 0.66 & 0.35 \\ 
  2020-07-01 & 0.68 & 0.63 & 0.55 & 0.58 & 0.40 & 0.71 & 0.40 \\ 
  2020-08-04 & 0.71 & 0.63 & 0.55 & 0.32 & 0.46 & 0.57 & 0.30 \\ 
  2020-09-02 & 0.52 & 0.63 & 0.52 & 0.18 & 0.42 & 0.49 & 0.31 \\ 
  2020-10-05 & 0.49 & 0.65 & 0.58 & 0.27 & 0.48 & 0.56 & 0.31 \\ 
  2020-11-03 & 0.58 & 0.55 & 0.50 & 0.30 & 0.50 & 0.51 & 0.27 \\ 
  2020-12-04 & 0.42 & 0.23 & 0.50 & 0.49 & 0.47 & 0.34 & 0.40 \\ 
  2021-01-14 & 0.36 & 0.46 & 0.55 & 0.16 & 0.46 & 0.52 & 0.42 \\ 
  2021-02-11 & 0.31 & 0.34 & 0.52 & 0.37 & 0.40 & 0.41 & 0.33 \\ 
  2021-03-11 & 0.42 & 0.40 & 0.51 & 0.34 & 0.42 & 0.34 & 0.29 \\ 
  2021-04-08 & 0.30 & 0.44 & 0.50 & 0.42 & 0.45 & 0.39 & 0.31 \\ 
  2021-05-06 & 0.28 & 0.34 & 0.45 & 0.31 & 0.36 & 0.35 & 0.39 \\ 
  2021-06-03 & 0.35 & 0.34 & 0.46 & 0.36 & 0.39 & 0.31 & 0.41 \\ 
  2021-07-01 & 0.30 & 0.29 & 0.41 & 0.27 & 0.36 & 0.31 & 0.39 \\ 
  2021-07-29 & 0.43 & 0.33 & 0.45 & 0.30 & 0.36 & 0.27 & 0.45 \\ 
  2021-08-26 & 0.43 & 0.31 & 0.40 & 0.26 & 0.32 & 0.25 & 0.47 \\ 
  2021-09-23 & 0.64 & 0.35 & 0.51 & 0.41 & 0.36 & 0.32 & 0.44 \\ 
  2021-10-22 & 0.14 & 0.38 & 0.47 & 0.32 & 0.37 & 0.26 & 0.43 \\ 
  2021-11-19 & 0.14 & 0.33 & 0.47 & 0.30 & 0.40 & 0.29 & 0.43 \\ 
  2022-01-03 & 0.14 & 0.36 & 0.41 & 0.40 & 0.36 & 0.33 & 0.42 \\ 
  2022-01-31 & 0.14 & 0.46 & 0.58 & 0.52 & 0.44 & 0.40 & 0.57 \\ 
  2022-02-28 & 0.79 & 0.57 & 0.62 & 0.52 & 0.55 & 0.61 & 0.64 \\ 
  2022-03-28 & 0.77 & 0.60 & 0.57 & 0.69 & 0.58 & 0.60 & 0.70 \\ 
  2022-04-28 & 0.84 & 0.86 & 0.85 & 0.93 & 0.84 & 0.89 & 0.90 \\ 
  2022-05-27 & 0.65 & 0.83 & 0.82 & 0.82 & 0.79 & 0.81 & 0.83 \\ 
  2022-06-28 & 0.94 & 0.84 & 0.84 & 0.82 & 0.85 & 0.84 & 0.85 \\ 
  2022-07-28 & 0.75 & 0.65 & 0.65 & 0.53 & 0.57 & 0.61 & 0.67 \\ 
  2022-08-25 & 0.60 & 0.50 & 0.57 & 0.38 & 0.50 & 0.42 & 0.60 \\ 
  2022-09-22 & 0.89 & 0.73 & 0.74 & 0.74 & 0.70 & 0.74 & 0.75 \\ 
  2022-10-20 & 0.94 & 0.75 & 0.75 & 0.76 & 0.76 & 0.76 & 0.81 \\ 
  2022-11-17 & 0.40 & 0.58 & 0.54 & 0.49 & 0.65 & 0.38 & 0.72 \\ 
  2023-01-04 & 0.48 & 0.48 & 0.57 & 0.47 & 0.50 & 0.29 & 0.59 \\ 
  2023-02-01 & 0.30 & 0.37 & 0.44 & 0.32 & 0.46 & 0.28 & 0.48 \\ 
  2023-03-01 & 0.48 & 0.33 & 0.44 & 0.31 & 0.39 & 0.32 & 0.46 \\ 
  2023-03-29 & 0.69 & 0.51 & 0.66 & 0.64 & 0.62 & 0.60 & 0.52 \\
   \hline
\end{tabular}
}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Expected shortfall for U.S.\ banks.}
\scalebox{0.8}{
\begin{tabular}{rrrrrrrr}
  \hline
 & AXP & BAC & C & GS & JPM & MS & WFC \\ 
  \hline
2019-02-28 & 45.58 & 78.22 & 92.27 & 120.89 & 77.42 & 110.05 & 75.51 \\ 
  2019-03-28 & 49.51 & 72.79 & 89.14 & 111.70 & 72.45 & 147.57 & 70.50 \\ 
  2019-04-26 & 46.32 & 77.45 & 89.56 & 116.14 & 77.33 & 118.48 & 74.59 \\ 
  2019-05-29 & 45.07 & 96.42 & 113.04 & 104.43 & 70.29 & 120.01 & 90.29 \\ 
  2019-06-26 & 39.27 & 104.44 & 120.68 & 104.19 & 67.55 & 113.41 & 95.57 \\ 
  2019-07-29 & 38.80 & 82.17 & 86.39 & 103.69 & 56.59 & 177.11 & 100.09 \\ 
  2019-09-10 & 41.10 & 86.03 & 87.80 & 105.08 & 83.97 & 126.69 & 85.05 \\ 
  2019-10-08 & 47.76 & 89.97 & 96.73 & 115.95 & 76.82 & 121.85 & 84.92 \\ 
  2019-11-06 & 38.45 & 88.76 & 84.54 & 102.49 & 72.61 & 117.70 & 76.72 \\ 
  2019-12-09 & 36.70 & 75.09 & 81.12 & 90.60 & 79.95 & 126.41 & 92.07 \\ 
  2020-01-13 & 40.95 & 74.41 & 75.35 & 100.54 & 69.26 & 118.86 & 73.45 \\ 
  2020-02-11 & 33.29 & 65.51 & 76.80 & 80.71 & 63.51 & 103.97 & 74.60 \\ 
  2020-03-11 & 58.69 & 141.30 & 162.90 & 146.33 & 133.54 & 178.94 & 141.11 \\ 
  2020-04-08 & 71.37 & 105.02 & 115.79 & 117.77 & 88.10 & 116.71 & 98.69 \\ 
  2020-05-06 & 60.15 & 78.49 & 102.32 & 109.76 & 79.31 & 94.44 & 84.64 \\ 
  2020-06-03 & 43.06 & 90.08 & 97.83 & 104.98 & 81.89 & 90.79 & 102.10 \\ 
  2020-07-01 & 32.43 & 82.84 & 94.93 & 106.72 & 88.40 & 84.01 & 94.59 \\ 
  2020-08-04 & 29.75 & 71.42 & 82.62 & 147.81 & 70.07 & 81.04 & 90.68 \\ 
  2020-09-02 & 31.94 & 61.63 & 74.73 & 333.48 & 69.03 & 71.80 & 85.74 \\ 
  2020-10-05 & 37.02 & 66.37 & 78.26 & 178.51 & 68.21 & 76.89 & 88.17 \\ 
  2020-11-03 & 37.32 & 70.52 & 83.12 & 186.00 & 64.82 & 77.48 & 94.10 \\ 
  2020-12-04 & 36.40 & 188.75 & 73.74 & 83.74 & 64.66 & 145.21 & 80.66 \\ 
  2021-01-14 & 42.02 & 66.68 & 68.93 & 499.93 & 68.62 & 70.96 & 77.39 \\ 
  2021-02-11 & 41.44 & 80.61 & 76.29 & 131.31 & 80.32 & 86.66 & 87.16 \\ 
  2021-03-11 & 39.96 & 75.14 & 76.94 & 134.97 & 72.03 & 103.86 & 87.01 \\ 
  2021-04-08 & 43.62 & 76.38 & 84.43 & 113.53 & 70.28 & 96.17 & 87.41 \\ 
  2021-05-06 & 41.72 & 78.62 & 81.94 & 139.54 & 79.91 & 91.23 & 77.38 \\ 
  2021-06-03 & 40.31 & 80.13 & 82.35 & 128.71 & 72.81 & 106.05 & 73.44 \\ 
  2021-07-01 & 40.79 & 81.20 & 80.40 & 165.81 & 67.16 & 93.29 & 71.51 \\ 
  2021-07-29 & 38.90 & 78.03 & 81.07 & 145.92 & 77.34 & 110.33 & 68.47 \\ 
  2021-08-26 & 37.98 & 75.12 & 79.14 & 153.11 & 79.11 & 101.72 & 63.16 \\ 
  2021-09-23 & 38.13 & 89.36 & 81.41 & 122.28 & 82.44 & 126.27 & 77.14 \\ 
  2021-10-22 & 36.45 & 73.18 & 81.63 & 133.22 & 76.29 & 124.90 & 72.95 \\ 
  2021-11-19 & 34.22 & 77.12 & 83.24 & 152.42 & 69.82 & 104.43 & 72.47 \\ 
  2022-01-03 & 34.38 & 85.00 & 95.48 & 108.55 & 80.01 & 98.31 & 81.79 \\ 
  2022-01-31 & 36.64 & 84.96 & 87.76 & 103.69 & 79.56 & 127.61 & 78.35 \\ 
  2022-02-28 & 35.53 & 81.80 & 90.67 & 119.44 & 77.66 & 90.70 & 81.59 \\ 
  2022-03-28 & 41.71 & 84.83 & 104.51 & 104.00 & 80.11 & 98.38 & 81.64 \\ 
  2022-04-28 & 51.16 & 91.84 & 108.28 & 109.53 & 87.30 & 105.31 & 88.08 \\ 
  2022-05-27 & 54.26 & 96.55 & 110.92 & 113.43 & 93.34 & 110.03 & 94.88 \\ 
  2022-06-28 & 51.47 & 115.31 & 131.55 & 135.27 & 107.09 & 128.79 & 109.22 \\ 
  2022-07-28 & 44.28 & 103.07 & 119.08 & 126.90 & 99.74 & 117.34 & 98.73 \\ 
  2022-08-25 & 44.16 & 103.30 & 115.73 & 132.86 & 97.13 & 150.50 & 95.11 \\ 
  2022-09-22 & 46.78 & 117.21 & 133.09 & 129.74 & 110.95 & 132.28 & 110.45 \\ 
  2022-10-20 & 44.55 & 120.48 & 138.81 & 140.68 & 110.10 & 137.93 & 110.64 \\ 
  2022-11-17 & 52.41 & 108.33 & 128.74 & 133.40 & 95.75 & 161.23 & 96.20 \\ 
  2023-01-04 & 46.78 & 112.63 & 122.95 & 130.01 & 103.76 & 227.25 & 101.35 \\ 
  2023-02-01 & 43.78 & 114.36 & 124.58 & 161.91 & 102.46 & 165.82 & 95.61 \\ 
  2023-03-01 & 40.92 & 115.97 & 122.14 & 156.62 & 108.11 & 127.51 & 94.15 \\ 
  2023-03-29 & 44.95 & 140.80 & 138.73 & 129.33 & 111.92 & 133.77 & 129.78 \\ 
   \hline
\end{tabular}
}
\end{table}

% EU
\begin{table}[!htbp] 
\centering
\caption{Probability of Distress for European banks.} 
\scalebox{0.8}{
\begin{tabular}{rrrrrrrrr}
  \hline
 & BCS & BNP & CS & GLE & ISP & SAN & UBS & UCG \\ 
  \hline
2019-02-28 & 0.01 & 0.01 & 0.00 & 0.00 & 0.05 & 0.00 & 0.00 & 0.01 \\ 
  2019-03-28 & 0.01 & 0.01 & 0.01 & 0.01 & 0.13 & 0.00 & 0.00 & 0.05 \\ 
  2019-04-26 & 0.00 & 0.00 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.01 \\ 
  2019-05-29 & 0.01 & 0.01 & 0.00 & 0.01 & 0.33 & 0.00 & 0.00 & 0.05 \\ 
  2019-06-26 & 0.00 & 0.01 & 0.00 & 0.00 & 0.05 & 0.00 & 0.00 & 0.01 \\ 
  2019-07-29 & 0.01 & 0.00 & 0.00 & 0.02 & 0.01 & 0.00 & 0.00 & 0.01 \\ 
  2019-09-10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2019-10-08 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2019-11-06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-12-09 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-01-13 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-02-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-03-11 & 0.04 & 0.21 & 0.26 & 0.20 & 0.40 & 0.04 & 0.15 & 0.31 \\ 
  2020-04-08 & 0.62 & 0.14 & 0.32 & 0.15 & 0.24 & 0.01 & 0.20 & 0.14 \\ 
  2020-05-06 & 0.30 & 0.05 & 0.02 & 0.05 & 0.22 & 0.00 & 0.15 & 0.14 \\ 
  2020-06-03 & 0.07 & 0.01 & 0.01 & 0.01 & 0.02 & 0.00 & 0.01 & 0.01 \\ 
  2020-07-01 & 0.03 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 \\ 
  2020-08-04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 \\ 
  2020-09-02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-10-05 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 \\ 
  2020-11-03 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-12-04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-01-14 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2021-02-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-03-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-04-08 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-05-06 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 \\ 
  2021-06-03 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-29 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-08-26 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-09-23 & 0.00 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-10-22 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-11-19 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-31 & 0.00 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.02 & 0.00 \\ 
  2022-02-28 & 0.00 & 0.08 & 0.41 & 0.17 & 0.00 & 0.03 & 0.36 & 0.01 \\ 
  2022-03-28 & 0.02 & 0.08 & 0.80 & 0.30 & 0.00 & 0.03 & 0.60 & 0.02 \\ 
  2022-04-28 & 0.05 & 0.11 & 0.81 & 0.26 & 0.04 & 0.03 & 0.44 & 0.01 \\ 
  2022-05-27 & 0.05 & 0.11 & 0.74 & 0.24 & 0.01 & 0.03 & 0.43 & 0.01 \\ 
  2022-06-28 & 0.79 & 0.54 & 0.98 & 0.77 & 0.01 & 0.12 & 0.96 & 0.04 \\ 
  2022-07-28 & 0.59 & 0.43 & 0.98 & 0.61 & 0.02 & 0.53 & 0.90 & 0.13 \\ 
  2022-08-25 & 0.57 & 0.21 & 0.99 & 0.28 & 0.00 & 0.49 & 0.84 & 0.02 \\ 
  2022-09-22 & 0.73 & 0.79 & 0.72 & 0.83 & 0.02 & 0.80 & 0.94 & 0.11 \\ 
  2022-10-20 & 0.82 & 0.87 & 0.81 & 0.90 & 0.01 & 0.88 & 0.97 & 0.06 \\ 
  2022-11-17 & 0.52 & 0.15 & 0.95 & 0.16 & 0.01 & 0.24 & 0.61 & 0.01 \\ 
  2023-01-04 & 0.03 & 0.04 & 0.98 & 0.05 & 0.00 & 0.02 & 0.22 & 0.00 \\ 
  2023-02-01 & 0.01 & 0.01 & 0.36 & 0.02 & 0.00 & 0.05 & 0.05 & 0.00 \\ 
  2023-03-01 & 0.00 & 0.00 & 0.69 & 0.01 & 0.00 & 0.01 & 0.02 & 0.00 \\ 
  2023-03-29 & 0.56 & 0.41 & 0.24 & 0.68 & 0.05 & 0.24 & 0.86 & 0.09 \\ 
   \hline
\end{tabular}
}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Joint Probability of Distress for European banks.} 
\scalebox{0.8}{
\begin{tabular}{rrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\ 
  \hline
2019-02-28 & 0.06 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-03-28 & 0.14 & 0.05 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-04-26 & 0.04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-05-29 & 0.33 & 0.06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-06-26 & 0.05 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-07-29 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-09-10 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-10-08 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-11-06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-12-09 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-01-13 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-02-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-03-11 & 0.56 & 0.40 & 0.27 & 0.18 & 0.11 & 0.06 & 0.03 & 0.01 \\ 
  2020-04-08 & 0.72 & 0.42 & 0.27 & 0.18 & 0.11 & 0.07 & 0.03 & 0.00 \\ 
  2020-05-06 & 0.43 & 0.23 & 0.14 & 0.07 & 0.04 & 0.02 & 0.01 & 0.00 \\ 
  2020-06-03 & 0.09 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-07-01 & 0.06 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-08-04 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-09-02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-10-05 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-11-03 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-12-04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-01-14 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-02-11 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-03-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-04-08 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-05-06 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-06-03 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-29 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-08-26 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-09-23 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-10-22 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-11-19 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-31 & 0.04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-02-28 & 0.55 & 0.30 & 0.14 & 0.06 & 0.02 & 0.00 & 0.00 & 0.00 \\ 
  2022-03-28 & 0.85 & 0.59 & 0.27 & 0.09 & 0.03 & 0.01 & 0.00 & 0.00 \\ 
  2022-04-28 & 0.84 & 0.49 & 0.24 & 0.11 & 0.05 & 0.02 & 0.01 & 0.00 \\ 
  2022-05-27 & 0.78 & 0.46 & 0.22 & 0.10 & 0.04 & 0.02 & 0.01 & 0.00 \\ 
  2022-06-28 & 0.99 & 0.97 & 0.88 & 0.72 & 0.49 & 0.12 & 0.03 & 0.01 \\ 
  2022-07-28 & 0.99 & 0.93 & 0.77 & 0.61 & 0.47 & 0.31 & 0.10 & 0.01 \\ 
  2022-08-25 & 0.99 & 0.89 & 0.65 & 0.44 & 0.27 & 0.14 & 0.01 & 0.00 \\ 
  2022-09-22 & 0.98 & 0.93 & 0.87 & 0.81 & 0.71 & 0.53 & 0.11 & 0.02 \\ 
  2022-10-20 & 0.99 & 0.97 & 0.93 & 0.89 & 0.82 & 0.66 & 0.06 & 0.01 \\ 
  2022-11-17 & 0.96 & 0.73 & 0.47 & 0.25 & 0.15 & 0.07 & 0.01 & 0.00 \\ 
  2023-01-04 & 0.98 & 0.24 & 0.07 & 0.03 & 0.01 & 0.01 & 0.00 & 0.00 \\ 
  2023-02-01 & 0.37 & 0.08 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-03-01 & 0.70 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-03-29 & 0.92 & 0.75 & 0.57 & 0.40 & 0.26 & 0.14 & 0.06 & 0.02 \\ 
   \hline
\end{tabular}
}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Expected proportion in Distress for European banks.}
\scalebox{0.8}{
\begin{tabular}{rrrrrrrrr}
  \hline
 & BCS & BNP & CS & GLE & ISP & SAN & UBS & UCG \\ 
  \hline
2019-02-28 & 0.28 & 0.37 & 0.39 & 0.38 & 0.18 & 0.25 & 0.44 & 0.31 \\ 
  2019-03-28 & 0.36 & 0.40 & 0.38 & 0.46 & 0.20 & 0.50 & 0.45 & 0.29 \\ 
  2019-04-26 & 0.28 & 0.36 & 0.28 & 0.42 & 0.17 & 0.12 & 0.46 & 0.29 \\ 
  2019-05-29 & 0.31 & 0.45 & 0.41 & 0.44 & 0.15 & 0.38 & 0.44 & 0.29 \\ 
  2019-06-26 & 0.28 & 0.29 & 0.35 & 0.46 & 0.17 & 0.12 & 0.38 & 0.30 \\ 
  2019-07-29 & 0.23 & 0.41 & 0.45 & 0.18 & 0.26 & 0.12 & 0.39 & 0.33 \\ 
  2019-09-10 & 0.18 & 0.24 & 0.26 & 0.33 & 0.22 & 0.12 & 0.28 & 0.32 \\ 
  2019-10-08 & 0.23 & 0.27 & 0.29 & 0.36 & 0.23 & 0.12 & 0.29 & 0.33 \\ 
  2019-11-06 & 0.17 & 0.23 & 0.19 & 0.27 & 0.22 & 0.12 & 0.17 & 0.29 \\ 
  2019-12-09 & 0.20 & 0.25 & 0.18 & 0.31 & 0.20 & 0.12 & 0.33 & 0.31 \\ 
  2020-01-13 & 0.17 & 0.21 & 0.12 & 0.38 & 0.20 & 0.12 & 0.12 & 0.30 \\ 
  2020-02-11 & 0.25 & 0.27 & 0.12 & 0.28 & 0.23 & 0.12 & 0.12 & 0.28 \\ 
  2020-03-11 & 0.64 & 0.55 & 0.48 & 0.56 & 0.43 & 0.78 & 0.54 & 0.48 \\ 
  2020-04-08 & 0.33 & 0.62 & 0.46 & 0.61 & 0.54 & 0.91 & 0.52 & 0.64 \\ 
  2020-05-06 & 0.30 & 0.56 & 0.64 & 0.57 & 0.38 & 0.79 & 0.39 & 0.46 \\ 
  2020-06-03 & 0.18 & 0.37 & 0.36 & 0.43 & 0.36 & 0.50 & 0.30 & 0.41 \\ 
  2020-07-01 & 0.21 & 0.35 & 0.34 & 0.40 & 0.34 & 0.57 & 0.27 & 0.40 \\ 
  2020-08-04 & 0.22 & 0.29 & 0.34 & 0.40 & 0.34 & 0.44 & 0.28 & 0.46 \\ 
  2020-09-02 & 0.16 & 0.21 & 0.12 & 0.31 & 0.28 & 0.12 & 0.20 & 0.33 \\ 
  2020-10-05 & 0.19 & 0.31 & 0.37 & 0.39 & 0.42 & 0.49 & 0.26 & 0.44 \\ 
  2020-11-03 & 0.17 & 0.32 & 0.33 & 0.41 & 0.47 & 0.41 & 0.30 & 0.42 \\ 
  2020-12-04 & 0.18 & 0.24 & 0.44 & 0.38 & 0.32 & 0.44 & 0.28 & 0.45 \\ 
  2021-01-14 & 0.22 & 0.41 & 0.44 & 0.44 & 0.24 & 0.44 & 0.30 & 0.33 \\ 
  2021-02-11 & 0.18 & 0.33 & 0.12 & 0.33 & 0.32 & 0.44 & 0.22 & 0.34 \\ 
  2021-03-11 & 0.21 & 0.27 & 0.22 & 0.29 & 0.38 & 0.20 & 0.18 & 0.28 \\ 
  2021-04-08 & 0.26 & 0.26 & 0.16 & 0.33 & 0.65 & 0.40 & 0.22 & 0.54 \\ 
  2021-05-06 & 0.27 & 0.24 & 0.28 & 0.28 & 0.54 & 0.34 & 0.20 & 0.49 \\ 
  2021-06-03 & 0.24 & 0.23 & 0.23 & 0.26 & 0.67 & 0.33 & 0.19 & 0.41 \\ 
  2021-07-01 & 0.18 & 0.23 & 0.22 & 0.23 & 0.12 & 0.17 & 0.19 & 0.34 \\ 
  2021-07-29 & 0.22 & 0.20 & 0.18 & 0.22 & 0.38 & 0.17 & 0.17 & 0.12 \\ 
  2021-08-26 & 0.17 & 0.17 & 0.13 & 0.18 & 0.12 & 0.12 & 0.12 & 0.12 \\ 
  2021-09-23 & 0.28 & 0.26 & 0.21 & 0.30 & 0.41 & 0.27 & 0.26 & 0.41 \\ 
  2021-10-22 & 0.23 & 0.21 & 0.19 & 0.26 & 0.50 & 0.22 & 0.20 & 0.12 \\ 
  2021-11-19 & 0.20 & 0.23 & 0.25 & 0.26 & 0.50 & 0.25 & 0.30 & 0.12 \\ 
  2022-01-03 & 0.32 & 0.25 & 0.20 & 0.26 & 0.39 & 0.29 & 0.23 & 0.53 \\ 
  2022-01-31 & 0.37 & 0.28 & 0.23 & 0.29 & 0.38 & 0.42 & 0.18 & 0.65 \\ 
  2022-02-28 & 0.64 & 0.49 & 0.28 & 0.39 & 0.75 & 0.57 & 0.29 & 0.65 \\ 
  2022-03-28 & 0.61 & 0.55 & 0.28 & 0.41 & 0.81 & 0.62 & 0.32 & 0.67 \\ 
  2022-04-28 & 0.58 & 0.56 & 0.27 & 0.44 & 0.63 & 0.68 & 0.36 & 0.79 \\ 
  2022-05-27 & 0.55 & 0.54 & 0.27 & 0.43 & 0.78 & 0.66 & 0.35 & 0.73 \\ 
  2022-06-28 & 0.58 & 0.65 & 0.53 & 0.59 & 0.93 & 0.77 & 0.54 & 0.85 \\ 
  2022-07-28 & 0.66 & 0.73 & 0.53 & 0.67 & 0.96 & 0.69 & 0.56 & 0.85 \\ 
  2022-08-25 & 0.55 & 0.70 & 0.43 & 0.67 & 0.92 & 0.58 & 0.47 & 0.85 \\ 
  2022-09-22 & 0.71 & 0.70 & 0.72 & 0.69 & 0.97 & 0.70 & 0.64 & 0.88 \\ 
  2022-10-20 & 0.72 & 0.71 & 0.72 & 0.71 & 0.98 & 0.71 & 0.68 & 0.90 \\ 
  2022-11-17 & 0.46 & 0.66 & 0.35 & 0.65 & 0.86 & 0.59 & 0.44 & 0.87 \\ 
  2023-01-04 & 0.48 & 0.49 & 0.17 & 0.47 & 0.73 & 0.58 & 0.31 & 0.69 \\ 
  2023-02-01 & 0.42 & 0.50 & 0.17 & 0.44 & 0.78 & 0.33 & 0.32 & 0.63 \\ 
  2023-03-01 & 0.44 & 0.50 & 0.13 & 0.40 & 0.69 & 0.38 & 0.30 & 0.73 \\ 
  2023-03-29 & 0.54 & 0.62 & 0.69 & 0.51 & 0.88 & 0.70 & 0.44 & 0.83 \\
   \hline
\end{tabular}
}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Expected shortfall for European banks.}
\scalebox{0.8}{
\begin{tabular}{rrrrrrrrr}
  \hline
 & BCS & BNP & CS & GLE & ISP & SAN & UBS & UCG \\ 
  \hline
2019-02-28 & 113.17 & 96.05 & 92.93 & 85.11 & 259.09 & 80.02 & 44.27 & 240.24 \\ 
  2019-03-28 & 99.61 & 77.84 & 112.16 & 71.96 & 246.78 & 88.10 & 48.52 & 252.60 \\ 
  2019-04-26 & 100.32 & 76.45 & 91.49 & 68.66 & 280.45 & 70.97 & 41.60 & 262.92 \\ 
  2019-05-29 & 112.56 & 69.56 & 98.65 & 69.18 & 287.30 & 64.96 & 35.12 & 239.98 \\ 
  2019-06-26 & 96.15 & 104.59 & 87.56 & 58.80 & 269.34 & 57.03 & 39.08 & 248.84 \\ 
  2019-07-29 & 115.97 & 97.54 & 80.49 & 245.12 & 233.97 & 55.41 & 43.08 & 242.71 \\ 
  2019-09-10 & 151.59 & 118.46 & 86.02 & 103.40 & 302.84 & 56.38 & 45.49 & 244.98 \\ 
  2019-10-08 & 122.15 & 122.91 & 101.95 & 85.82 & 273.34 & 63.88 & 50.56 & 241.28 \\ 
  2019-11-06 & 172.03 & 132.31 & 76.41 & 108.80 & 286.41 & 58.67 & 42.50 & 231.22 \\ 
  2019-12-09 & 108.08 & 148.12 & 135.74 & 90.80 & 280.65 & 45.03 & 57.78 & 205.09 \\ 
  2020-01-13 & 83.90 & 209.25 & 60.96 & 89.15 & 300.35 & 43.85 & 33.83 & 248.17 \\ 
  2020-02-11 & 156.79 & 236.15 & 72.92 & 117.24 & 229.51 & 40.74 & 32.83 & 263.39 \\ 
  2020-03-11 & 88.09 & 115.14 & 209.08 & 103.88 & 283.72 & 98.24 & 78.22 & 269.96 \\ 
  2020-04-08 & 140.29 & 87.94 & 163.46 & 87.90 & 208.07 & 85.95 & 73.39 & 194.25 \\ 
  2020-05-06 & 125.05 & 83.23 & 119.15 & 81.52 & 216.35 & 82.95 & 72.02 & 213.20 \\ 
  2020-06-03 & 130.20 & 94.71 & 128.73 & 85.78 & 224.12 & 72.85 & 64.59 & 208.04 \\ 
  2020-07-01 & 116.69 & 97.13 & 126.03 & 86.30 & 213.19 & 80.91 & 65.84 & 205.24 \\ 
  2020-08-04 & 119.62 & 112.13 & 107.90 & 87.23 & 261.74 & 88.71 & 60.31 & 191.75 \\ 
  2020-09-02 & 151.16 & 175.40 & 60.95 & 104.45 & 234.10 & 65.21 & 41.12 & 188.00 \\ 
  2020-10-05 & 126.54 & 142.96 & 101.55 & 103.56 & 232.21 & 79.86 & 68.65 & 206.43 \\ 
  2020-11-03 & 130.88 & 127.64 & 102.73 & 97.40 & 203.97 & 89.04 & 51.61 & 193.53 \\ 
  2020-12-04 & 146.06 & 136.42 & 77.76 & 94.42 & 352.27 & 57.98 & 48.85 & 171.83 \\ 
  2021-01-14 & 108.08 & 84.13 & 75.59 & 72.89 & 370.94 & 64.16 & 50.36 & 221.51 \\ 
  2021-02-11 & 164.76 & 116.19 & 66.62 & 105.32 & 308.33 & 70.76 & 47.84 & 202.33 \\ 
  2021-03-11 & 101.79 & 107.88 & 73.42 & 96.78 & 191.86 & 63.58 & 41.44 & 162.96 \\ 
  2021-04-08 & 88.01 & 103.83 & 158.78 & 75.32 & 122.17 & 61.72 & 47.54 & 126.50 \\ 
  2021-05-06 & 99.67 & 103.63 & 87.11 & 87.80 & 126.38 & 59.77 & 49.20 & 138.08 \\ 
  2021-06-03 & 89.31 & 112.11 & 98.98 & 90.82 & 114.92 & 56.60 & 44.90 & 140.70 \\ 
  2021-07-01 & 69.23 & 82.91 & 97.20 & 89.65 & 111.59 & 54.94 & 46.40 & 129.36 \\ 
  2021-07-29 & 107.61 & 156.54 & 96.13 & 86.10 & 108.43 & 50.25 & 38.22 & 116.59 \\ 
  2021-08-26 & 154.27 & 249.09 & 88.88 & 79.62 & 92.30 & 41.29 & 32.93 & 86.10 \\ 
  2021-09-23 & 83.08 & 94.65 & 127.28 & 81.44 & 162.37 & 71.28 & 45.26 & 139.07 \\ 
  2021-10-22 & 105.53 & 141.14 & 106.95 & 84.36 & 124.17 & 61.25 & 42.75 & 103.42 \\ 
  2021-11-19 & 79.45 & 78.23 & 93.03 & 85.19 & 145.96 & 65.73 & 44.26 & 119.62 \\ 
  2022-01-03 & 98.78 & 128.06 & 116.25 & 90.05 & 184.22 & 62.67 & 51.08 & 131.20 \\ 
  2022-01-31 & 82.29 & 86.98 & 113.92 & 76.82 & 171.65 & 60.21 & 56.24 & 114.75 \\ 
  2022-02-28 & 67.88 & 64.41 & 137.91 & 79.05 & 89.64 & 60.08 & 59.46 & 116.66 \\ 
  2022-03-28 & 74.55 & 58.43 & 140.37 & 73.22 & 93.94 & 59.14 & 66.00 & 121.75 \\ 
  2022-04-28 & 84.11 & 63.40 & 146.99 & 72.58 & 140.50 & 61.34 & 62.54 & 137.53 \\ 
  2022-05-27 & 87.55 & 64.45 & 148.26 & 73.31 & 136.85 & 60.34 & 64.55 & 139.47 \\ 
  2022-06-28 & 119.96 & 72.60 & 198.65 & 80.25 & 138.57 & 66.46 & 76.67 & 149.40 \\ 
  2022-07-28 & 114.03 & 72.20 & 211.08 & 81.37 & 141.00 & 81.75 & 75.95 & 161.91 \\ 
  2022-08-25 & 113.12 & 67.15 & 217.61 & 73.73 & 122.85 & 80.04 & 75.70 & 146.99 \\ 
  2022-09-22 & 133.88 & 83.98 & 227.65 & 91.89 & 144.29 & 93.84 & 96.86 & 168.30 \\ 
  2022-10-20 & 141.34 & 90.32 & 300.53 & 107.01 & 142.27 & 95.38 & 116.23 & 160.06 \\ 
  2022-11-17 & 133.70 & 69.81 & 422.44 & 77.86 & 125.03 & 81.13 & 91.36 & 135.62 \\ 
  2023-01-04 & 110.81 & 68.87 & 477.80 & 77.09 & 119.01 & 70.50 & 89.88 & 126.99 \\ 
  2023-02-01 & 112.24 & 65.52 & 403.00 & 75.97 & 110.24 & 85.02 & 83.75 & 126.15 \\ 
  2023-03-01 & 102.40 & 60.41 & 500.92 & 73.51 & 106.69 & 74.93 & 85.73 & 111.56 \\ 
  2023-03-29 & 164.92 & 85.47 & 377.30 & 113.14 & 124.69 & 81.95 & 159.20 & 135.08 \\ 
   \hline
\end{tabular}
}
\end{table}

% All

\begin{table}[!htbp] 
\centering
\caption{Probability of Distress for U.S.\ and European banks.} 
\scalebox{0.8}{
\begin{tabular}{rrrrrrrrrrrrrrrr}
  \hline
 & BCS & BNP & CS & GLE & ISP & SAN & UBS & UCG & AXP & BAC & C & GS & JPM & MS & WFC \\ 
  \hline
2019-02-28 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.05 \\ 
  2019-03-28 & 0.00 & 0.01 & 0.00 & 0.00 & 0.15 & 0.00 & 0.00 & 0.06 & 0.02 & 0.00 & 0.00 & 0.01 & 0.00 & 0.13 & 0.07 \\ 
  2019-04-26 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\ 
  2019-05-29 & 0.01 & 0.00 & 0.00 & 0.00 & 0.39 & 0.00 & 0.00 & 0.03 & 0.02 & 0.05 & 0.08 & 0.03 & 0.01 & 0.08 & 0.44 \\ 
  2019-06-26 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.07 \\ 
  2019-07-29 & 0.00 & 0.00 & 0.00 & 0.06 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.03 \\ 
  2019-09-10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-10-08 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.01 & 0.02 & 0.01 & 0.01 & 0.15 \\ 
  2019-11-06 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-12-09 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-01-13 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-02-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-03-11 & 0.09 & 0.33 & 0.34 & 0.33 & 0.46 & 0.10 & 0.22 & 0.41 & 0.53 & 0.48 & 0.56 & 0.55 & 0.63 & 0.58 & 0.64 \\ 
  2020-04-08 & 0.59 & 0.17 & 0.37 & 0.22 & 0.32 & 0.00 & 0.26 & 0.20 & 0.78 & 0.50 & 0.62 & 0.53 & 0.59 & 0.47 & 0.83 \\ 
  2020-05-06 & 0.31 & 0.03 & 0.01 & 0.03 & 0.23 & 0.00 & 0.17 & 0.15 & 0.42 & 0.13 & 0.48 & 0.30 & 0.44 & 0.18 & 0.49 \\ 
  2020-06-03 & 0.07 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.07 & 0.08 & 0.10 & 0.08 & 0.18 & 0.03 & 0.30 \\ 
  2020-07-01 & 0.03 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.02 & 0.14 & 0.22 & 0.18 & 0.36 & 0.06 & 0.40 \\ 
  2020-08-04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.17 & 0.03 & 0.01 & 0.17 \\ 
  2020-09-02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.18 & 0.00 & 0.00 & 0.01 \\ 
  2020-10-05 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.25 & 0.03 & 0.01 & 0.14 \\ 
  2020-11-03 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.10 & 0.01 & 0.00 & 0.11 \\ 
  2020-12-04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 \\ 
  2021-01-14 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.37 & 0.00 & 0.00 & 0.00 \\ 
  2021-02-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-03-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\ 
  2021-04-08 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.02 \\ 
  2021-05-06 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2021-06-03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-29 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2021-08-26 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-09-23 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.01 & 0.02 & 0.03 & 0.01 \\ 
  2021-10-22 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 \\ 
  2021-11-19 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 \\ 
  2022-01-31 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.19 & 0.10 & 0.11 & 0.21 & 0.26 & 0.10 \\ 
  2022-02-28 & 0.00 & 0.11 & 0.45 & 0.23 & 0.00 & 0.02 & 0.39 & 0.00 & 0.00 & 0.37 & 0.30 & 0.42 & 0.39 & 0.25 & 0.28 \\ 
  2022-03-28 & 0.02 & 0.09 & 0.78 & 0.34 & 0.00 & 0.02 & 0.58 & 0.01 & 0.05 & 0.47 & 0.51 & 0.26 & 0.49 & 0.40 & 0.32 \\ 
  2022-04-28 & 0.06 & 0.11 & 0.80 & 0.30 & 0.06 & 0.02 & 0.44 & 0.00 & 0.78 & 0.82 & 0.83 & 0.59 & 0.87 & 0.73 & 0.72 \\ 
  2022-05-27 & 0.05 & 0.10 & 0.75 & 0.27 & 0.00 & 0.02 & 0.44 & 0.00 & 0.82 & 0.56 & 0.57 & 0.51 & 0.61 & 0.53 & 0.55 \\ 
  2022-06-28 & 0.74 & 0.56 & 0.99 & 0.77 & 0.00 & 0.13 & 0.96 & 0.04 & 0.33 & 0.80 & 0.82 & 0.80 & 0.78 & 0.78 & 0.78 \\ 
  2022-07-28 & 0.58 & 0.46 & 0.98 & 0.61 & 0.01 & 0.55 & 0.89 & 0.15 & 0.03 & 0.35 & 0.35 & 0.44 & 0.44 & 0.31 & 0.30 \\ 
  2022-08-25 & 0.57 & 0.21 & 0.99 & 0.28 & 0.00 & 0.51 & 0.84 & 0.01 & 0.00 & 0.08 & 0.06 & 0.15 & 0.09 & 0.19 & 0.04 \\ 
  2022-09-22 & 0.70 & 0.77 & 0.70 & 0.82 & 0.01 & 0.78 & 0.93 & 0.12 & 0.11 & 0.65 & 0.63 & 0.58 & 0.68 & 0.56 & 0.62 \\ 
  2022-10-20 & 0.78 & 0.86 & 0.76 & 0.86 & 0.00 & 0.86 & 0.97 & 0.05 & 0.03 & 0.83 & 0.82 & 0.75 & 0.77 & 0.75 & 0.65 \\ 
  2022-11-17 & 0.52 & 0.18 & 0.92 & 0.20 & 0.00 & 0.27 & 0.59 & 0.00 & 0.18 & 0.08 & 0.14 & 0.11 & 0.06 & 0.32 & 0.04 \\ 
  2023-01-04 & 0.03 & 0.03 & 0.98 & 0.03 & 0.00 & 0.00 & 0.25 & 0.00 & 0.01 & 0.07 & 0.04 & 0.04 & 0.08 & 0.31 & 0.04 \\ 
  2023-02-01 & 0.01 & 0.00 & 0.39 & 0.00 & 0.00 & 0.04 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 \\ 
  2023-03-01 & 0.00 & 0.00 & 0.69 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-03-29 & 0.56 & 0.44 & 0.33 & 0.65 & 0.07 & 0.28 & 0.82 & 0.11 & 0.04 & 0.48 & 0.32 & 0.26 & 0.33 & 0.29 & 0.44 \\ 
   \hline
\end{tabular}}
\end{table}

\begin{table}[!htbp] 
\caption{Joint Probability of Distress for U.S.\ and European banks.} 
\centering
\scalebox{0.8}{
\begin{tabular}{rrrrrrrrrrrrrrrr}
  \hline
 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 \\ 
  \hline
2019-02-28 & 0.07 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-03-28 & 0.28 & 0.12 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-04-26 & 0.04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-05-29 & 0.64 & 0.28 & 0.11 & 0.06 & 0.03 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-06-26 & 0.09 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-07-29 & 0.08 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-09-10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-10-08 & 0.17 & 0.04 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-11-06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2019-12-09 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-01-13 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-02-11 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-03-11 & 0.93 & 0.86 & 0.78 & 0.72 & 0.65 & 0.57 & 0.48 & 0.37 & 0.29 & 0.23 & 0.16 & 0.11 & 0.07 & 0.03 & 0.01 \\ 
  2020-04-08 & 0.97 & 0.91 & 0.84 & 0.76 & 0.68 & 0.60 & 0.51 & 0.39 & 0.29 & 0.22 & 0.15 & 0.10 & 0.06 & 0.03 & 0.00 \\ 
  2020-05-06 & 0.80 & 0.66 & 0.53 & 0.42 & 0.32 & 0.23 & 0.16 & 0.10 & 0.06 & 0.04 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 \\ 
  2020-06-03 & 0.40 & 0.22 & 0.13 & 0.08 & 0.05 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-07-01 & 0.53 & 0.35 & 0.23 & 0.15 & 0.09 & 0.04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-08-04 & 0.26 & 0.11 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-09-02 & 0.19 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-10-05 & 0.30 & 0.11 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-11-03 & 0.18 & 0.06 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2020-12-04 & 0.11 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-01-14 & 0.37 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-02-11 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-03-11 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-04-08 & 0.06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-05-06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-06-03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-07-29 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-08-26 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-09-23 & 0.06 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-10-22 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2021-11-19 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-03 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-01-31 & 0.40 & 0.24 & 0.15 & 0.10 & 0.06 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-02-28 & 0.80 & 0.64 & 0.52 & 0.41 & 0.31 & 0.23 & 0.15 & 0.09 & 0.04 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2022-03-28 & 0.91 & 0.79 & 0.65 & 0.54 & 0.45 & 0.36 & 0.27 & 0.19 & 0.11 & 0.05 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2022-04-28 & 0.98 & 0.95 & 0.92 & 0.87 & 0.81 & 0.75 & 0.65 & 0.52 & 0.34 & 0.19 & 0.09 & 0.04 & 0.01 & 0.00 & 0.00 \\ 
  2022-05-27 & 0.96 & 0.88 & 0.79 & 0.70 & 0.63 & 0.55 & 0.46 & 0.36 & 0.24 & 0.13 & 0.06 & 0.02 & 0.01 & 0.00 & 0.00 \\ 
  2022-06-28 & 1.00 & 0.99 & 0.98 & 0.95 & 0.92 & 0.87 & 0.82 & 0.77 & 0.68 & 0.57 & 0.42 & 0.22 & 0.07 & 0.01 & 0.00 \\ 
  2022-07-28 & 0.99 & 0.95 & 0.86 & 0.77 & 0.66 & 0.56 & 0.46 & 0.37 & 0.29 & 0.22 & 0.16 & 0.10 & 0.04 & 0.01 & 0.00 \\ 
  2022-08-25 & 1.00 & 0.90 & 0.71 & 0.53 & 0.36 & 0.23 & 0.13 & 0.07 & 0.05 & 0.03 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2022-09-22 & 0.99 & 0.97 & 0.94 & 0.90 & 0.85 & 0.80 & 0.72 & 0.64 & 0.57 & 0.49 & 0.39 & 0.27 & 0.11 & 0.02 & 0.00 \\ 
  2022-10-20 & 1.00 & 0.99 & 0.98 & 0.96 & 0.94 & 0.91 & 0.85 & 0.79 & 0.72 & 0.64 & 0.53 & 0.36 & 0.06 & 0.01 & 0.00 \\ 
  2022-11-17 & 0.95 & 0.78 & 0.60 & 0.43 & 0.31 & 0.21 & 0.14 & 0.09 & 0.05 & 0.03 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 \\ 
  2023-01-04 & 0.98 & 0.47 & 0.21 & 0.11 & 0.06 & 0.04 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-02-01 & 0.40 & 0.07 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-03-01 & 0.69 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2023-03-29 & 0.93 & 0.83 & 0.74 & 0.65 & 0.54 & 0.45 & 0.35 & 0.28 & 0.21 & 0.16 & 0.12 & 0.08 & 0.05 & 0.02 & 0.01 \\ 
   \hline
\end{tabular}}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Expected Proportion in Distress for U.S.\ and European banks.}
\scalebox{0.8}{
\begin{tabular}{rrrrrrrrrrrrrrrr}
  \hline
 & BCS & BNP & CS & GLE & ISP & SAN & UBS & UCG & AXP & BAC & C & GS & JPM & MS & WFC \\  
  \hline
2019-02-28 & 0.13 & 0.20 & 0.07 & 0.27 & 0.08 & 0.07 & 0.07 & 0.19 & 0.14 & 0.07 & 0.20 & 0.14 & 0.19 & 0.21 & 0.08 \\ 
  2019-03-28 & 0.21 & 0.35 & 0.27 & 0.42 & 0.12 & 0.07 & 0.30 & 0.17 & 0.18 & 0.34 & 0.33 & 0.25 & 0.30 & 0.13 & 0.16 \\ 
  2019-04-26 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.13 & 0.11 & 0.07 & 0.23 & 0.16 & 0.20 & 0.19 & 0.10 \\ 
  2019-05-29 & 0.26 & 0.45 & 0.07 & 0.43 & 0.13 & 0.07 & 0.07 & 0.21 & 0.31 & 0.31 & 0.27 & 0.33 & 0.36 & 0.27 & 0.14 \\ 
  2019-06-26 & 0.07 & 0.18 & 0.07 & 0.07 & 0.08 & 0.07 & 0.07 & 0.17 & 0.16 & 0.20 & 0.17 & 0.23 & 0.26 & 0.21 & 0.08 \\ 
  2019-07-29 & 0.15 & 0.07 & 0.07 & 0.09 & 0.18 & 0.07 & 0.07 & 0.19 & 0.20 & 0.24 & 0.23 & 0.23 & 0.07 & 0.15 & 0.11 \\ 
  2019-09-10 & 0.08 & 0.07 & 0.07 & 0.07 & 0.09 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.13 & 0.13 & 0.07 & 0.10 \\ 
  2019-10-08 & 0.08 & 0.23 & 0.07 & 0.07 & 0.10 & 0.07 & 0.07 & 0.07 & 0.16 & 0.32 & 0.28 & 0.19 & 0.23 & 0.21 & 0.09 \\ 
  2019-11-06 & 0.07 & 0.07 & 0.07 & 0.07 & 0.09 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.20 & 0.20 & 0.07 & 0.13 \\ 
  2019-12-09 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.10 & 0.07 & 0.13 \\ 
  2020-01-13 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.15 & 0.07 & 0.10 \\ 
  2020-02-11 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.09 \\ 
  2020-03-11 & 0.70 & 0.62 & 0.62 & 0.62 & 0.58 & 0.77 & 0.65 & 0.60 & 0.55 & 0.59 & 0.56 & 0.57 & 0.53 & 0.56 & 0.53 \\ 
  2020-04-08 & 0.53 & 0.70 & 0.61 & 0.67 & 0.64 & 0.92 & 0.63 & 0.69 & 0.49 & 0.58 & 0.55 & 0.59 & 0.55 & 0.60 & 0.49 \\ 
  2020-05-06 & 0.38 & 0.69 & 0.71 & 0.71 & 0.40 & 0.84 & 0.43 & 0.45 & 0.35 & 0.53 & 0.36 & 0.43 & 0.37 & 0.48 & 0.36 \\ 
  2020-06-03 & 0.20 & 0.43 & 0.43 & 0.48 & 0.29 & 0.07 & 0.31 & 0.32 & 0.26 & 0.30 & 0.28 & 0.29 & 0.22 & 0.34 & 0.17 \\ 
  2020-07-01 & 0.28 & 0.49 & 0.43 & 0.51 & 0.33 & 0.07 & 0.34 & 0.42 & 0.38 & 0.31 & 0.27 & 0.29 & 0.21 & 0.36 & 0.21 \\ 
  2020-08-04 & 0.15 & 0.24 & 0.07 & 0.24 & 0.19 & 0.07 & 0.17 & 0.07 & 0.33 & 0.31 & 0.25 & 0.13 & 0.21 & 0.26 & 0.13 \\ 
  2020-09-02 & 0.08 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.16 & 0.07 & 0.07 & 0.07 & 0.15 & 0.07 & 0.14 \\ 
  2020-10-05 & 0.11 & 0.15 & 0.07 & 0.18 & 0.07 & 0.07 & 0.14 & 0.07 & 0.24 & 0.32 & 0.25 & 0.11 & 0.20 & 0.26 & 0.14 \\ 
  2020-11-03 & 0.10 & 0.15 & 0.07 & 0.18 & 0.07 & 0.07 & 0.12 & 0.07 & 0.20 & 0.25 & 0.21 & 0.12 & 0.24 & 0.27 & 0.11 \\ 
  2020-12-04 & 0.09 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.16 & 0.08 & 0.26 & 0.25 & 0.24 & 0.13 & 0.21 \\ 
  2021-01-14 & 0.11 & 0.07 & 0.07 & 0.07 & 0.14 & 0.07 & 0.17 & 0.20 & 0.14 & 0.17 & 0.07 & 0.07 & 0.16 & 0.07 & 0.18 \\ 
  2021-02-11 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.08 & 0.20 & 0.07 & 0.10 & 0.11 & 0.27 & 0.12 \\ 
  2021-03-11 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.11 & 0.19 & 0.27 & 0.13 & 0.19 & 0.14 & 0.11 \\ 
  2021-04-08 & 0.07 & 0.07 & 0.08 & 0.07 & 0.07 & 0.07 & 0.10 & 0.07 & 0.11 & 0.23 & 0.21 & 0.14 & 0.21 & 0.19 & 0.11 \\ 
  2021-05-06 & 0.07 & 0.13 & 0.07 & 0.17 & 0.07 & 0.07 & 0.09 & 0.07 & 0.08 & 0.18 & 0.17 & 0.09 & 0.12 & 0.07 & 0.22 \\ 
  2021-06-03 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.10 & 0.07 & 0.11 & 0.19 & 0.23 & 0.10 & 0.16 & 0.12 & 0.16 \\ 
  2021-07-01 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.08 & 0.07 & 0.23 & 0.07 \\ 
  2021-07-29 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.10 & 0.27 & 0.22 & 0.09 & 0.14 & 0.11 & 0.07 \\ 
  2021-08-26 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.09 & 0.07 & 0.07 & 0.08 & 0.13 & 0.09 & 0.07 \\ 
  2021-09-23 & 0.08 & 0.21 & 0.16 & 0.27 & 0.07 & 0.23 & 0.15 & 0.07 & 0.24 & 0.16 & 0.30 & 0.18 & 0.16 & 0.14 & 0.24 \\ 
  2021-10-22 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.24 & 0.21 & 0.10 & 0.17 & 0.10 & 0.33 \\ 
  2021-11-19 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.16 & 0.15 & 0.15 & 0.17 & 0.10 & 0.13 \\ 
  2022-01-03 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.08 & 0.07 & 0.07 & 0.14 & 0.15 & 0.21 & 0.13 & 0.16 & 0.19 \\ 
  2022-01-31 & 0.07 & 0.41 & 0.34 & 0.34 & 0.07 & 0.07 & 0.27 & 0.07 & 0.07 & 0.23 & 0.30 & 0.26 & 0.22 & 0.19 & 0.29 \\ 
  2022-02-28 & 0.52 & 0.44 & 0.33 & 0.37 & 0.07 & 0.62 & 0.34 & 0.77 & 0.63 & 0.38 & 0.41 & 0.35 & 0.37 & 0.41 & 0.41 \\ 
  2022-03-28 & 0.62 & 0.60 & 0.35 & 0.48 & 0.07 & 0.65 & 0.37 & 0.62 & 0.57 & 0.45 & 0.43 & 0.50 & 0.43 & 0.45 & 0.50 \\ 
  2022-04-28 & 0.72 & 0.71 & 0.52 & 0.63 & 0.72 & 0.80 & 0.59 & 0.86 & 0.52 & 0.53 & 0.53 & 0.58 & 0.52 & 0.55 & 0.56 \\ 
  2022-05-27 & 0.66 & 0.65 & 0.45 & 0.57 & 0.78 & 0.74 & 0.52 & 0.79 & 0.43 & 0.52 & 0.52 & 0.53 & 0.51 & 0.52 & 0.53 \\ 
  2022-06-28 & 0.68 & 0.71 & 0.62 & 0.67 & 0.89 & 0.81 & 0.63 & 0.86 & 0.75 & 0.68 & 0.68 & 0.68 & 0.69 & 0.68 & 0.69 \\ 
  2022-07-28 & 0.54 & 0.58 & 0.44 & 0.54 & 0.80 & 0.55 & 0.46 & 0.68 & 0.75 & 0.64 & 0.64 & 0.59 & 0.60 & 0.64 & 0.66 \\ 
  2022-08-25 & 0.35 & 0.45 & 0.27 & 0.42 & 0.73 & 0.36 & 0.30 & 0.61 & 0.62 & 0.55 & 0.59 & 0.47 & 0.52 & 0.45 & 0.62 \\ 
  2022-09-22 & 0.66 & 0.65 & 0.67 & 0.64 & 0.89 & 0.65 & 0.60 & 0.81 & 0.80 & 0.69 & 0.70 & 0.70 & 0.69 & 0.71 & 0.70 \\ 
  2022-10-20 & 0.70 & 0.69 & 0.71 & 0.69 & 0.94 & 0.69 & 0.66 & 0.87 & 0.85 & 0.70 & 0.71 & 0.71 & 0.72 & 0.71 & 0.74 \\ 
  2022-11-17 & 0.34 & 0.46 & 0.26 & 0.45 & 0.66 & 0.42 & 0.32 & 0.68 & 0.40 & 0.55 & 0.50 & 0.49 & 0.58 & 0.39 & 0.65 \\ 
  2023-01-04 & 0.34 & 0.35 & 0.13 & 0.34 & 0.60 & 0.48 & 0.22 & 0.65 & 0.36 & 0.35 & 0.40 & 0.35 & 0.34 & 0.22 & 0.39 \\ 
  2023-02-01 & 0.21 & 0.26 & 0.08 & 0.27 & 0.07 & 0.17 & 0.16 & 0.07 & 0.19 & 0.26 & 0.31 & 0.22 & 0.32 & 0.19 & 0.38 \\ 
  2023-03-01 & 0.23 & 0.07 & 0.07 & 0.30 & 0.07 & 0.20 & 0.15 & 0.07 & 0.07 & 0.23 & 0.33 & 0.22 & 0.21 & 0.19 & 0.33 \\ 
  2023-03-29 & 0.49 & 0.53 & 0.57 & 0.46 & 0.81 & 0.61 & 0.41 & 0.77 & 0.67 & 0.53 & 0.60 & 0.59 & 0.59 & 0.58 & 0.54 \\ 
   \hline
\end{tabular}
}
\end{table}

\begin{table}[!htbp] 
\centering
\caption{Expected Shortfall for U.S.\ and European banks.}
\scalebox{0.7}{
\begin{tabular}{rrrrrrrrrrrrrrrr}
  \hline
 & BCS & BNP & CS & GLE & ISP & SAN & UBS & UCG & AXP & BAC & C & GS & JPM & MS & WFC \\ 
  \hline
2019-02-28 & 80.06 & 68.66 & 81.84 & 68.77 & 170.90 & 65.69 & 37.87 & 156.14 & 43.32 & 68.89 & 80.22 & 109.45 & 71.31 & 91.37 & 68.34 \\ 
  2019-03-28 & 84.15 & 65.19 & 102.33 & 65.21 & 195.76 & 76.65 & 43.16 & 199.18 & 43.96 & 61.67 & 73.75 & 96.13 & 60.99 & 111.84 & 60.61 \\ 
  2019-04-26 & 73.07 & 54.87 & 83.70 & 57.41 & 187.45 & 59.04 & 37.73 & 172.10 & 43.46 & 63.47 & 72.78 & 100.84 & 64.70 & 86.13 & 61.55 \\ 
  2019-05-29 & 89.13 & 55.15 & 86.35 & 57.49 & 214.48 & 53.57 & 30.64 & 175.02 & 40.95 & 80.92 & 91.35 & 93.05 & 61.07 & 96.65 & 81.06 \\ 
  2019-06-26 & 68.36 & 71.07 & 76.51 & 47.52 & 166.58 & 45.21 & 31.56 & 147.36 & 38.55 & 90.30 & 94.87 & 92.05 & 60.31 & 85.50 & 80.82 \\ 
  2019-07-29 & 84.15 & 47.26 & 64.38 & 160.81 & 139.78 & 43.54 & 29.21 & 140.73 & 36.33 & 62.09 & 68.43 & 82.74 & 46.04 & 98.58 & 68.27 \\ 
  2019-09-10 & 85.23 & 39.68 & 51.62 & 51.02 & 113.95 & 40.41 & 26.38 & 101.64 & 41.93 & 67.10 & 73.20 & 93.15 & 84.77 & 90.37 & 68.79 \\ 
  2019-10-08 & 74.77 & 53.62 & 65.87 & 48.89 & 119.69 & 44.60 & 30.63 & 112.92 & 48.24 & 79.23 & 87.85 & 110.36 & 69.77 & 101.68 & 76.05 \\ 
  2019-11-06 & 113.82 & 61.20 & 59.87 & 70.70 & 132.08 & 42.54 & 31.35 & 112.14 & 33.00 & 62.29 & 65.86 & 83.85 & 66.65 & 75.34 & 60.56 \\ 
  2019-12-09 & 65.11 & 41.52 & 97.63 & 49.95 & 114.30 & 39.48 & 39.89 & 89.91 & 36.96 & 81.95 & 70.69 & 124.41 & 85.06 & 91.45 & 68.51 \\ 
  2020-01-13 & 51.31 & 35.26 & 46.72 & 38.69 & 96.75 & 32.67 & 25.93 & 86.95 & 38.93 & 73.65 & 73.81 & 103.17 & 91.90 & 86.84 & 76.96 \\ 
  2020-02-11 & 60.23 & 41.80 & 61.01 & 49.96 & 80.82 & 34.40 & 27.48 & 71.47 & 34.28 & 64.88 & 66.85 & 83.45 & 74.48 & 72.84 & 74.10 \\ 
  2020-03-11 & 79.70 & 96.52 & 150.05 & 96.16 & 251.83 & 82.42 & 60.00 & 235.43 & 56.86 & 146.36 & 165.27 & 150.29 & 144.11 & 180.19 & 159.17 \\ 
  2020-04-08 & 127.14 & 76.44 & 139.26 & 77.46 & 179.41 & 76.14 & 63.54 & 170.76 & 70.16 & 103.45 & 115.55 & 117.68 & 89.62 & 114.06 & 98.47 \\ 
  2020-05-06 & 111.82 & 71.33 & 106.87 & 71.33 & 180.32 & 71.59 & 63.67 & 178.51 & 55.70 & 75.28 & 98.73 & 106.45 & 76.39 & 90.91 & 80.57 \\ 
  2020-06-03 & 96.49 & 55.85 & 78.30 & 56.06 & 125.04 & 52.42 & 45.38 & 125.14 & 40.11 & 79.72 & 89.34 & 100.52 & 76.79 & 80.46 & 90.82 \\ 
  2020-07-01 & 82.97 & 54.38 & 78.81 & 55.62 & 120.33 & 53.25 & 44.87 & 121.87 & 31.85 & 79.83 & 92.27 & 103.99 & 86.13 & 80.88 & 90.48 \\ 
  2020-08-04 & 76.47 & 55.23 & 69.32 & 52.07 & 102.88 & 56.85 & 41.55 & 107.86 & 28.90 & 66.24 & 77.16 & 133.46 & 64.81 & 74.48 & 83.21 \\ 
  2020-09-02 & 65.67 & 41.52 & 50.83 & 41.50 & 83.09 & 44.24 & 33.62 & 79.84 & 32.22 & 56.09 & 70.53 & 339.79 & 62.96 & 68.65 & 76.95 \\ 
  2020-10-05 & 69.62 & 42.02 & 56.00 & 42.32 & 100.32 & 51.35 & 36.29 & 105.03 & 36.30 & 61.59 & 73.42 & 156.78 & 62.96 & 69.63 & 82.79 \\ 
  2020-11-03 & 75.39 & 43.69 & 58.87 & 44.02 & 104.23 & 55.84 & 31.80 & 113.26 & 36.27 & 62.02 & 74.84 & 149.15 & 58.17 & 66.68 & 85.22 \\ 
  2020-12-04 & 62.99 & 43.09 & 52.14 & 41.39 & 68.41 & 38.78 & 30.70 & 74.31 & 36.68 & 138.64 & 63.94 & 67.25 & 53.06 & 106.60 & 67.27 \\ 
  2021-01-14 & 66.33 & 40.52 & 55.75 & 39.81 & 159.30 & 49.10 & 35.96 & 127.94 & 41.53 & 55.11 & 59.04 & 459.75 & 58.60 & 57.72 & 63.97 \\ 
  2021-02-11 & 51.69 & 32.51 & 46.11 & 33.16 & 64.07 & 36.55 & 29.18 & 67.10 & 42.41 & 63.32 & 69.12 & 165.33 & 76.37 & 96.29 & 72.56 \\ 
  2021-03-11 & 47.44 & 29.04 & 47.27 & 27.90 & 70.86 & 39.31 & 29.13 & 76.92 & 39.03 & 68.97 & 72.46 & 115.94 & 68.11 & 84.07 & 76.97 \\ 
  2021-04-08 & 52.72 & 40.15 & 86.29 & 38.35 & 74.82 & 43.14 & 36.43 & 81.61 & 43.10 & 65.18 & 75.09 & 131.27 & 61.84 & 80.11 & 79.07 \\ 
  2021-05-06 & 59.56 & 50.33 & 68.10 & 51.49 & 74.32 & 47.44 & 41.71 & 82.91 & 41.14 & 64.25 & 69.15 & 205.48 & 66.32 & 69.45 & 63.35 \\ 
  2021-06-03 & 50.23 & 41.98 & 68.10 & 43.39 & 68.53 & 38.57 & 37.42 & 75.75 & 39.43 & 66.59 & 75.05 & 168.84 & 65.68 & 118.43 & 65.54 \\ 
  2021-07-01 & 46.11 & 39.16 & 61.64 & 40.08 & 59.20 & 31.95 & 35.37 & 69.44 & 41.11 & 64.71 & 80.41 & 235.23 & 58.41 & 159.71 & 60.67 \\ 
  2021-07-29 & 44.54 & 36.54 & 62.47 & 37.82 & 56.09 & 33.54 & 33.05 & 61.07 & 38.56 & 63.78 & 74.33 & 171.58 & 66.09 & 133.03 & 60.94 \\ 
  2021-08-26 & 44.90 & 36.34 & 59.30 & 35.31 & 55.78 & 31.52 & 31.89 & 61.79 & 37.06 & 63.86 & 74.07 & 191.63 & 68.83 & 160.44 & 56.12 \\ 
  2021-09-23 & 53.45 & 46.18 & 75.90 & 44.63 & 69.73 & 42.48 & 36.48 & 74.54 & 37.49 & 76.61 & 73.57 & 95.62 & 71.93 & 112.41 & 67.65 \\ 
  2021-10-22 & 48.22 & 35.69 & 59.52 & 35.65 & 63.19 & 40.17 & 36.02 & 69.57 & 36.57 & 66.08 & 74.95 & 182.98 & 66.03 & 99.43 & 64.90 \\ 
  2021-11-19 & 52.20 & 41.81 & 64.29 & 45.48 & 68.85 & 42.38 & 36.23 & 78.27 & 34.23 & 70.49 & 83.01 & 90.08 & 67.37 & 136.99 & 69.52 \\ 
  2022-01-03 & 58.94 & 41.06 & 66.59 & 43.94 & 68.32 & 42.30 & 36.21 & 72.75 & 34.53 & 78.03 & 89.50 & 83.57 & 72.54 & 80.54 & 73.04 \\ 
  2022-01-31 & 58.80 & 42.54 & 76.12 & 45.37 & 79.49 & 44.22 & 43.35 & 77.65 & 36.53 & 79.76 & 83.13 & 96.97 & 75.07 & 111.45 & 74.03 \\ 
  2022-02-28 & 63.73 & 54.07 & 117.36 & 64.68 & 81.52 & 52.99 & 53.83 & 105.56 & 34.65 & 75.91 & 84.47 & 113.90 & 71.78 & 84.76 & 74.99 \\ 
  2022-03-28 & 72.42 & 55.84 & 134.26 & 69.94 & 89.50 & 56.54 & 62.92 & 115.15 & 40.81 & 79.27 & 97.32 & 97.96 & 75.04 & 92.26 & 76.40 \\ 
  2022-04-28 & 78.64 & 57.59 & 135.14 & 65.87 & 119.65 & 56.24 & 58.10 & 128.42 & 51.06 & 91.00 & 107.47 & 107.97 & 86.58 & 104.09 & 87.45 \\ 
  2022-05-27 & 83.23 & 59.22 & 137.57 & 67.12 & 126.88 & 55.03 & 60.04 & 129.72 & 54.00 & 94.12 & 108.54 & 110.35 & 91.25 & 107.15 & 92.61 \\ 
  2022-06-28 & 119.42 & 72.02 & 196.60 & 79.61 & 137.46 & 66.06 & 76.10 & 148.53 & 51.29 & 112.42 & 128.80 & 132.43 & 104.79 & 125.54 & 106.89 \\ 
  2022-07-28 & 113.48 & 71.72 & 209.15 & 80.80 & 140.05 & 81.28 & 75.40 & 160.93 & 42.47 & 92.89 & 107.86 & 115.08 & 90.64 & 105.67 & 90.34 \\ 
  2022-08-25 & 112.62 & 66.77 & 215.82 & 73.20 & 122.04 & 79.71 & 75.25 & 146.46 & 41.34 & 82.35 & 93.21 & 104.23 & 79.39 & 89.02 & 79.26 \\ 
  2022-09-22 & 132.52 & 82.89 & 224.14 & 90.68 & 142.78 & 92.67 & 95.74 & 166.99 & 45.92 & 110.04 & 125.00 & 123.61 & 104.98 & 123.56 & 104.35 \\ 
  2022-10-20 & 140.36 & 89.54 & 295.89 & 105.85 & 141.30 & 94.64 & 115.01 & 159.31 & 44.13 & 117.08 & 135.22 & 136.35 & 107.33 & 133.82 & 107.99 \\ 
  2022-11-17 & 132.39 & 68.80 & 416.78 & 76.89 & 123.49 & 80.19 & 89.87 & 134.26 & 47.93 & 90.75 & 108.85 & 112.15 & 82.70 & 117.87 & 83.30 \\ 
  2023-01-04 & 105.04 & 63.62 & 429.12 & 70.73 & 113.97 & 66.71 & 81.43 & 121.98 & 44.50 & 93.00 & 102.93 & 106.32 & 85.22 & 146.36 & 85.40 \\ 
  2023-02-01 & 109.58 & 62.44 & 379.62 & 71.13 & 107.64 & 82.45 & 81.12 & 123.33 & 40.30 & 77.67 & 85.76 & 91.39 & 71.04 & 88.02 & 72.07 \\ 
  2023-03-01 & 98.67 & 56.53 & 441.79 & 65.25 & 103.76 & 69.27 & 82.13 & 110.19 & 39.04 & 84.06 & 91.70 & 96.87 & 78.42 & 87.92 & 76.46 \\ 
  2023-03-29 & 160.57 & 82.51 & 403.48 & 109.72 & 123.01 & 79.46 & 155.98 & 131.92 & 43.20 & 119.17 & 116.78 & 116.61 & 94.84 & 113.39 & 108.86 \\ 
   \hline
\end{tabular}
}
\end{table}


